Aerial Shepherds: Enabling Hierarchical Localization in Heterogeneous MAV Swarms

A heterogeneous micro aerial vehicles (MAV) swarm consists of resource-intensive but expensive advanced MAVs (AMAVs) and resource-limited but cost-effective basic MAVs (BMAVs), offering opportunities in diverse fields. Accurate and real-time localization is crucial for MAV swarms, but current practices lack a low-cost, high-precision, and real-time solution, especially for lightweight BMAVs. We find an opportunity to accomplish the task by transforming AMAVs into mobile localization infrastructures for BMAVs. However, translating this insight into a practical system is challenging due to issues in estimating locations with diverse and unknown localization errors of BMAVs, and allocating resources of AMAVs considering interconnected influential factors. This work introduces TransformLoc, a new framework that transforms AMAVs into mobile localization infrastructures, specifically designed for low-cost and resource-constrained BMAVs. We design an error-aware joint location estimation model to perform intermittent joint estimation for BMAVs and introduce a similarity-instructed adaptive grouping-scheduling strategy to allocate resources of AMAVs dynamically. TransformLoc achieves a collaborative, adaptive, and cost-effective localization system suitable for large-scale heterogeneous MAV swarms. We implement and validate TransformLoc on industrial drones. Results show it outperforms all baselines by up to 68\% in localization performance, improving navigation success rates by 60\%. Extensive robustness and ablation experiments further highlight the superiority of its design.

==> evaluation_backup.tex <==
\section{Evaluation}\label{5}
% In this section, we evaluate the performance of \textit{H-Swarm} in location estimation and navigation for BMAVs through real experiments on a real heterogeneous MAV swarm testbed and physical feature-based simulation.
\begin{figure*}[t]
    \centering
        \includegraphics[width=1.6\columnwidth]{Figs/setup.pdf}
    \caption{The real-world heterogeneous MAV swarm implementation and experiment area. We collect noise models from this heterogeneous MAV swarm. The AMAV utilizes a T265 tracking camera to localize itself and a logi C310 RGB camera to generate observation for BMAVs. The Pixhawk open-source controller and ArduPilot open-source flight control framework control the motion of the AMAV. The BMAV is acted by crazyfile mounted an AprilTag for recognition and localization. The ground truth is obtained from OptiTrack cameras. The experiment area is 8m * 8m square area.}
    \label{setup}
    % \vspace{-0.4cm}
\end{figure*} 
In this section, we evaluate the performance of \textit{H-Swarm} in localization and navigation of BMAVs through large-scale physical feature-based simulation with the noise models collected from a real heterogeneous MAV swarm testbed.
The evaluation focus on the following aspects:
\begin{itemize}
    % \item Validating the assumptions of the physical-feature-based simulation experiments through the real heterogeneous MAV swarm testbed experiments.
    \item Characterizing the performance of the \textit{H-Swarm} in terms of (1) navigation duration and success rate and (2) average error of location estimations of BMAVs in comparison to existing methods.  
    \item Testing the robustness of the \textit{H-Swarm} with changing parameters, such as the number of BMAVs and AMAVs, the noise of motion and observation sensors, and the search tree pruning parameters.
\end{itemize}

We first introduce the evaluation metrics and baselines in Section \ref{5.1}. 
% Then, the setup of the real heterogeneous MAV swarm testbed are described in Section \ref{5.2}.
% Subsequently, the detail of experiments on a real heterogeneous MAV swarm testbed is presented in Section \ref{5.3}. 
The settings of the physical-featured-based simulation environment are described in Section \ref{5.4}.
Several large-scale physical-featured-based simulations are conducted to illustrate the overall performance of the system in Section \ref{5.5}.
Finally, we validate the system’s robustness in diverse system parameter settings in Section \ref{5.6}.

\subsection{Evaluation Metrics and Baselines} \label{5.1}
\subsubsection{Evaluation Metrics} 
Our \textit{H-Swarm} system aims to limit the localization error of BMAVs and improve the navigation success rate of BMAVs. Therefore, two metrics are introduced to evaluate the performance of the system:

\textbf{Localization error: } \textit{H-Swarm} will report the 2D location estimation of BMAVs at each timestep during the navigation. We compare the reported location estimation with the ground truth of BMAVs to calculate the localization error of BMAVs, which is Absolute Trajectory Error, (ATE).

\textbf{Success rate: } The BAMVs aim to navigate to pre-determined destinations to sense the environment. Therefore, we measure the success rate of BMAVs' navigation by counting the ratio of BMAVs which reach the destination within a limited time and with limited destination accuracy.

\subsubsection{Baselines} 
We compare our \textit{H-Swarm} with two baselines that do not require any location infrastructure to validate the advantages of our system.

\textbf{Dead Reckoning:}\cite{borenstein1996navigating} Dead reckoning is an infrastructure-free technique used to estimate the BMAV's location. This method utilizes noisy measurements from motion sensors of BMAVs, to estimate the location change of BMAVs. Then the BMAVs use the location estimation to navigate to destinations similar to \textit{H-Swarm}.

\textbf{Station:}\cite{xu2020learning} Station is an infrastructure-free technique that utilizes AMAVs with fixed locations to generate observations for BMAVs. The locations of AMAVs are generated by the dispersion algorithm \cite{purohit2013sugarmap}. The observations are then adopted to correct the localization error of BMAVs. The navigation strategy of BMAVs is similar to \textit{H-Swarm}.

% \subsection{Testbed Experiment Setup} \label{5.2}
% \begin{figure*}[t]
%     \centering
%         \includegraphics[width=1.6\columnwidth]{Figs/setup.pdf}
%     \caption{Architecture of the sensing system, which is composed of four subsystems.}
%     \label{setup}
%     % \vspace{-0.4cm}
% \end{figure*} 
% To build the prototype of the \textit{H-Swarm} for the validation in real world, we implement our system on the Crazyfile (A commercial micro unmanned aerial vehicle) and ArduPilot (A widely-used open source drone flight control framework). The implementation detail consists of four parts.

% \textbf{AMAV platform: }

% \textbf{BMAV platform: }

% \textbf{Ground station: }

% \textbf{Ground truth acquisition: }

% \subsection{Testbed Experiment Results}\label{5.3}

\subsection{Physical Feature Based Simulation Environment} \label{5.4}

\subsubsection{Noise model collected from real-world} We collect motion noise model and observation model from real-world heterogeneous MAV swarm implementation as illustrated in Fig. \ref{setup}. The AMAV is equipped with a T265 tracking camera for localization and a logi C310 RGB camera to generate observation. Meanwhile, the AMAV utilizes Pixhawk open-source controller and ArduPilot open-source flight control framework to control the motion of the AMAV. The BMAV is acted by crazyfile, which mounted an AprilTag that enabled AMAV to recognize and generate observations for it. Multiple OptiTrack cameras working at 240 FPS are deployed in the experiment area to obtain millimeter-level ground truth.

\subsubsection{The heterogeneous MAV swarm simulator}
We implemented a heterogeneous MAV swarm simulator to evaluate our \textit{H-Swarm} system at a large scale. The simulator includes a realistic physical arena, noise models of different sensors collected from the testbed described above, and motion models of AMAV and BMAV. we set the simulation time-step is 1$sec$ to evaluate our system as follows:
% and configured the simulator

\textbf{Arena:} We use an indoor scenario similar to Fig. \ref{setup} (b). The BMAVs navigate to different destinations and the AMAVs travel to generate observations for BMAVs. In more complex environments, the BMAVs need to be equipped with obstacle avoidance modules to complete more complex navigation, which will be completed in future work. 

\textbf{BMAV sensors and mobility:} The sensors on BMAV in the simulation are modeled after the Crazyfile platform.
% , which also served as BMAV in the testbed experiments. 
Each BMAV has a gyroscope, an optical flow sensor, and an ultrasonic altitude measurement sensor. The noise model of motion is obtained through empirical measurements of the real-world swarm. The maximum velocity of BMAV is set to 0.5$m/s$ and the command interval $\delta$ is set to 5. 
% in accordance with the testbed parameters. 
The velocity of BMAV varies due to the noisiness of the optical flow sensor and the distance to the destination.

\textbf{AMAV sensors and mobility:} Each AMAV uses a tracking camera and SLAM algorithm to obtain its own location. At the same time, each AMAV also uses visual sensors to calibrate the localization error of BMAVs. The observation angle $\theta$ of the visual sensor is 120 degrees and the maximum observation distance $r_m$ is 1\textit{m}. The control commands of AMAV use motion primitives $\{(u, \omega)\}| u \in \{0, 1, 3\}m/s, \omega \in \{0, \pm1, \pm3\}rad/s$.

\textbf{Destination of BMAVs: }We have all BMAVs start from the bottom left corner of the room and spread out as much as possible to sense the environment. Therefore, the destination of BMAVs is at the edge of the room as shown in Fig. \ref{Demo}.

In the default setting, all the simulations are performed 10 times with 3 AMAVs and 9 BMAVs to evaluate both the performance and the robustness of the system. We set the standard deviation $\sigma$ of BMAV's motion noise model as 20\% of the measured velocity value for both the x and y-axis according to testbed measurement and \cite{chen2020h}. We set the standard deviation $\sigma$ of the range measurement noise model of AMAV as 10\% of the range measurement between the AMAV and BMAV, and the standard deviation $\sigma$ of the bearing measurement noise model of AMAV as 5\% of the angle measurement between the AMAV and BMAV according to testbed measurement and \cite{wang2016apriltag}. The search tree pruning parameter $\epsilon$ is set to 1 and $\sigma$ is set to 10. We run the simulation for a time period of 420 seconds (~7 minutes) corresponding to the typical battery life of Crazyfile \cite{preiss2017crazyswarm}.

\begin{figure*}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    \subfigure[Navigation success rate comparison]{
        \centering
            \includegraphics[width=0.63\columnwidth]{Figs/navDes.png}
        % \label{success100s}
    }
    \subfigure[Navigation success rate comparison]{
        \centering
            \includegraphics[width=0.63\columnwidth]{Figs/navtime.png}
        % \label{success0.2m}
    }
    \subfigure[Localization error comparison]{
        \centering
            \includegraphics[width=0.65\columnwidth]{Figs/meancdf.png}
        % \label{success0.2m}
    }
\caption{The overall performance of \textit{H-Swarm} in terms of navigation success rate and localization error. (a) The navigation success rate of \textit{H-Swarm} under different destination accuracy constraints within 100 seconds. (b) The navigation success rate as a function of time limitation under 0.2m destination accuracy constraint. (c) The cumulative distribution function (CDF) of location estimation errors from a typical run.}
\label{simOverall}
\end{figure*}

\subsection{System performance} \label{5.5}
The simulations in this section evaluate the navigation success rate of the BMAVs under different destination constraints and time constraints. In the meanwhile, the localization error of all BMAVs is evaluated.
% We measure the success rate of BMAVs' navigation by counting the number of BMAVs which reach the destination within a limited time and with limited destination accuracy.


\subsubsection{Success Rate VS Destination Accuracy} 
In order to validate the performance of \textit{H-Swarm} under different destination accuracy constraints, we evaluate the success rate of BMAVs' navigation given varies destination accuracy within 100 seconds as Fig. \ref{simOverall} (a) illustrated.
With the increase in destination accuracy, the navigation success rate of BMAVs using different methods increases. This is because the increase in destination accuracy means that the farther away the destination is when the BMAV is successfully navigated. 
For example, when the destination accuracy is 0.5m and the distance between BMAV and the destination is less than 0.5m, the navigation is considered successful.
% If the destination accuracy is 0.25m, the distance between the BMAV and the destination must be less than 0.25m before the navigation is successful.
The H-Swarm outperformed all baselines with different destination accuracy conditions. 
Specifically, when destination accuracy is strict (0.2m), \textit{H-Swarm} achieves an acceptable success rate of around 80\%, while all baselines are below 50\%. 
This means that under strict destination accuracy constraints, Station and Dead Reckoning cannot achieve efficient navigation within the time limitation, while \textit{H-Swarm}, with the help of mobile AMAVs, Still working.
For less constrained destination accuracy (0.4 to 0.6 m), \textit{H-Swarm} shows consistently a 30\% higher success rate than all baselines.
When the destination accuracy is looser (0.8m), \textit{H-Swarm} achieves a 100\% navigation success rate while all baselines are less than 80\%.
In summary, these results show that \textit{H-Swarm} can effectively deal with different destination accuracy and achieve a high success rate of navigation.

\subsubsection{Success Rate VS Time Limitation}
\begin{figure}[t]
    \centering
        \includegraphics[width=1\columnwidth]{Figs/Demo.pdf}
    \caption{The figure shows the demonstration of a typical run with 3 AMAVs and 9 BMAVs. At $t=0$, all BMAVs start from the lower left corner.
    % and arrive at destinations indicated by "x". 
    During the navigation, their localization errors and estimation uncertainty are increasing. \textit{H-Swarm} groups AMAVs and BMAVs reasonably to allocate sensing resources of AMAVs. Finally, all BMAVs reached destinations.}
    \label{Demo}
    % \vspace{-0.4cm}
\end{figure} 
In order to validate the performance of \textit{H-Swarm} under different time limitations, we evaluate the navigation success rate of BMAVs with different time limitations under 0.2m destination accuracy constraint as Fig. \ref{simOverall} (b) illustrated.
As time limitation increases, the navigation success rate of BMAVs for all methods increases because BMAVs have more time to close in on the destination.
The \textit{H-Swarm} outperforms other baselines in all time constraints.
Specifically, under strict time constraints (60-180 seconds), \textit{H-Swarm}'s navigation success rate is nearly 10\% higher than that of the Station. 
This is because, in the Station method, AMAVs are distributed at the locations that BMAVs will pass through, allowing AMAVs to generate observations for BMAVs. 
Under the relaxed time constraints (240-420 seconds), the \textit{H-Swarm} achieved a navigation success rate of 100\%, nearly 20\% more than the Station, and 40\% more than the Dead Reckoning. This is because \textit{H-Swarm} dispatches AMAVs to provide observations for BMAVs as they approach final destinations.
% helping to reduce localization errors.
Fig. \ref{Demo} provides a demonstration of the navigation process under 0.2m destination accuracy constraint of \textit{H-Swarm}. 
During the navigation, \textit{H-Swarm} navigates AMAVs appropriately and allocates sensing resources to BMAVs.
In conclusion, \textit{H-Swarm} can reasonably allocate sensing resources of AMAVs under different time constraints to provide observations for BMAVs and improve their navigation success rate.

\subsubsection{Localization Error}
\begin{figure}[t]
    \centering
        \includegraphics[width=0.98\columnwidth]{Figs/overallLoc.pdf}
    \caption{The figure shows the localization error of BMAVs and localization error on average in a typical run with 3 AMAVs and 9 BMAVs. When AMAV generates observations for BMAV, the localization error decreases significantly. For \textit{H-Swarm}, BMAVs' localization errors remained low, while for other methods, BMAVs' localization errors increased. This indicates that \textit{H-Swarm} can reasonably allocate sensing resources of AMAVs.}
    \label{localization}
    % \vspace{-0.4cm}
\end{figure} 
To further verify the localization performance of \textit{H-Swarm}, we control each BMAV to start an independent 420-second random walk from point (5,5). Figure \ref{simOverall} (c) illustrates the cumulative distribution function (CDF) of localization errors using three methods from a typical experiment.
With \textit{H-Swarm}, observations from moving AMAVs kept the localization error of BMAVs below 1 meter. In contrast, the localization error of the Station remained below 2.2 m, while that of the Dead Reckoning was below 3 m.
Fig. \ref{localization} illustrates the change of localization error and average localization error of different BMAVs in 420s. In the absence of AMAV observations, the localization error of BMAVs with three methods is the same. With \textit{H-Swarm}, the AMAVs started providing observations for BMAVs in the first 10 seconds, while Station could only provide observations if BMAVs were within the FoV. For example, in the random walk process of BMAV 2, \textit{H-Swarm} keeps its localization error below 1m, while Station's localization error is close to 5.5m, and Dead-Reckoning's is close to 7m.
In short, \textit{H-Swarm} is able to dispatch AMAVs to provide timely observations for BMAVs, keeping the localization error low.


\subsection{Influence of System Settings} \label{5.6}
In this section, we conduct experiments to investigate how different system parameters setting affect the performance of three methods.
% when BMAVs are random walking. 
Specifically, we check the variance on (1) the number of AMAVs and  BMAVs, (2) the noise of the motion measurement of BMAV, (3) the noise of range measurement, and (4) the parameter setting of the search tree.

\subsubsection{Number of AMAVs}
To evaluate how the number of AMAVs affects the localization error of BMAVs, we plot the average localization error of different methods against varying numbers of AMAVs as illustrated in Fig. \ref{AMAVnumber} (a).
The average BAMVs localization error of different methods decreases with the increase of the number of AMAVs, and after the introduction of AMAV, the localization error of BMAVs of \textit{H-Swarm} and Station is lower than that of Dead Reckoning.
This is because AMAVs can generate observations for BMAVs, helping to reduce localization errors. As the number of AMAVs increased, the average localization error of BMAVs of \textit{H-Swarm} gradually fell below 0.5 m, while that of Station remained above 1.5 m. 
This is because moving AMAVs in an \textit{H-Swarm} can generate more observations for BMAVs, helping to reduce localization errors, whereas Station can only help BMAVs reduce localization errors when they pass over AMAVs.
Fig. \ref{AMAVnumber} (b) shows The CDF of the average localization error of BMAVs with 5 AMAVs. The \textit{H-Swarm} consistently kept the average localization error below 1 m, while the Station and Dead Reckoning both recorded a maximum average location error of over 2 m.
In summary, experimental results show that the average localization error of BMAVs decreases significantly with the increase in the number of AMAVs.
\begin{figure}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    \subfigure[Localization error comparison]{
        \centering
            \includegraphics[width=0.52\columnwidth]{Figs/AMAV.png}
        % \label{success100s}
    }
    \subfigure[Localization error CDF]{
        \centering
            \includegraphics[width=0.39\columnwidth]{Figs/AMAVcdf.png}
        % \label{success0.2m}
    }
\caption{The figures show the localization error of BAMVs on average with different numbers of AMAVs and localization error CDF with five AMAVs. Due to the introduction of AMAV, the localization errors of BMAVs are reduced compared to the Dead Reckoning method. As the number of AMAVs increases, the average localization error of BMAVs decreases. The \textit{H-Swarm} always has a lower localization error.}
\label{AMAVnumber}
\end{figure}

\subsubsection{Number of BMAVs}
\begin{figure}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    \subfigure[Localization error comparison]{
        \centering
            \includegraphics[width=0.52\columnwidth]{Figs/BMAV.png}
        % \label{success100s}
    }
    \subfigure[Localization error CDF]{
        \centering
            \includegraphics[width=0.39\columnwidth]{Figs/BMAVcdf.png}
        % \label{success0.2m}
    }
\caption{The figures show the localization error of BAMVs on average with different numbers of BAMVs and localization error CDF with eleven BMAVs. As the number of BMAVs increases, the average localization error of BMAVs increases. The \textit{H-Swarm} always has a lower localization error.}
\label{BMAVnumber}
\end{figure}
In order to evaluate the effect of the number of BMAVs on localization errors, we plot the average localization errors against varying numbers of BMAVs as illustrated in Fig. \ref{BMAVnumber} (a).
With the increase in the number of BMAVs, the average localization error of BMAVs of different methods showed an increasing trend, because the number of BMAVs passing through AMAVs decreased with the increase of the number of BMAVs. 
With different numbers of BMAVs, the \textit{H-Swarm} has consistently achieved an average localization error of less than 1 meter, which is more than a 2x reduction than the average localization error of any other baselines.
This is because the system can reasonably allocate the sensing resources of AMAVs so that AMAVs can provide observations for different BMAVs.
Fig. \ref{BMAVnumber} (b) shows The CDF of the average localization error of BMAVs with eleven AMAVs.
The \textit{H-Swarm} consistently kept the average localization error below 2 m, while other methods recorded a maximum average location error of over 3 m.
The experimental results show that \textit{H-Swarm} can handle the situation of different numbers of BMAVs, which keeps the localization error at a low level.

\subsubsection{Motion measurement noise of BMAV}
\begin{figure}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    \subfigure[Localization error comparison]{
        \centering
            \includegraphics[width=0.52\columnwidth]{Figs/monoise.png}
        % \label{success100s}
    }
    \subfigure[Localization error CDF]{
        \centering
            \includegraphics[width=0.39\columnwidth]{Figs/monoisecdf.png}
        % \label{success0.2m}
    }
\caption{The figures show the localization error of BAMVs on average with different motion noise of BAMVs and localization error CDF with 30\% motion noise. The noise of the sensor is modeled as a normal distribution with varying standard deviations. As the motion noise standard deviation of BMAVs increases, the average localization error of BMAVs increases. The \textit{H-Swarm} always has a lower localization error.}
\label{MotionNoise}
\end{figure}
There is noise in BMAV motion measurements, which will gradually increase the localization error of BMAV. 
In addition, the greater the noise in motion measurements, the faster the growth rate of the localization error of BMAV. 
Therefore, this is an important parameter to determine the system's performance. In order to evaluate the performance of the \textit{H-Swarm} for varying levels of sensor noise, We plot localization error against varying motion measurement noise levels in Fig. \ref{MotionNoise} (a).
With the increase of motion measurement noise, the average localization error of BMAVs with different methods increases. The average localization error with \textit{H-Swarm} is significantly lower than that of other baselines. When the motion measurement noise increases to 30\%, the average localization error of Dead Reckoning reaches 2.5m, and that of Station reaches 2m. The \textit{H-Swarm} has an average localization error of less than one meter. This is due to the fact that \textit{H-Swarm} has the ability to allocate sensing resources of AMAVs in time to generate observations for BMAVs.
Fig. \ref{MotionNoise} (b) shows The CDF of the average localization error of BMAVs with 30\% motion measurement noise.
The \textit{H-Swarm} consistently kept the average localization error below 2 m, while the Station and Dead Reckoning both recorded a maximum average location error of over 3 m.
This result demonstrates the superior performance of \textit{H-Swarm}, particularly in large motion measurement noise.

\subsubsection{Range measurement noise of AMAV}
\begin{figure}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    \subfigure[Localization error comparison]{
        \centering
            \includegraphics[width=0.52\columnwidth]{Figs/obnoise.png}
        % \label{success100s}
    }
    \subfigure[Localization error CDF]{
        \centering
            \includegraphics[width=0.39\columnwidth]{Figs/obnoisecdf.png}
        % \label{success0.2m}
    }
\caption{The figures show the localization error of BAMVs on average with different range measurement noise of AMAVs and localization error CDF with 20\% range measurement noise. The noise of the sensor is modeled as a normal distribution with varying standard deviations. As the range measurement noise standard deviation, the average localization error of BMAVs increases. The\ \textit{H-Swarm} always has a lower localization error.}
\label{rangenoise}
\end{figure}
According to testbed's tests and \cite{kalaitzakis2021fiducial}, in the relative distance and angle measurement method based on AprilTag \cite{wang2016apriltag}, the error of relative angle measurement is lower, but the error of relative distance measurement can't be ignored. 
Therefore, the noise in range measurements due to visual sensors is an important parameter in determining the performance of the system.
In order to study the impact of range measurement noise on the \textit{H-Swarm}, we compared the average localization error of BMAVs under different noise conditions as Fig. \ref{rangenoise}(a) shows.
The results show that when the range measurement noise increases, the average localization errors of both \textit{H-Swarm} and Station increase. This is because the increase in range measurement noise causes the gap between the observations provided by AMAVs for BMAVs and the true locations of BMAVs to increase.
The \textit{H-Swarm} outperforms the baselines in different range measurement noise conditions. This is because \textit{H-Swarm} is able to plan AMAVs to provide observations for BMAVs at locations closer to BMAVs, reducing the impact of range measurement noise.
Fig. \ref{rangenoise}(b) shows the localization error CDF of the three methods when the range measurement noise is 20\%. The \textit{H-Swarm} is able to maintain an average localization error of fewer than 1.5 meters, while the other baselines have an average localization error of more than 2 meters. Experimental results show that the \textit{H-Swarm} is able to cope with a wide range of measurement noise.

\subsubsection{Search tree pruning parameter and runtime}
\begin{figure}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    % \subfigure[Alpha influence]{
    %     \centering
    %     % \label{success100s}
    % }
    % \subfigure[Beta influence]{
    %     \centering
    %         \includegraphics[width=0.46\columnwidth]{Figs/beta.png}
    %     % \label{success0.2m}
    % }
    \includegraphics[width=0.9\columnwidth]{Figs/alpha.pdf}
\caption{The figures show the localization error of BMAVs on average with different $\epsilon$ settings. As $\epsilon$ grows, fewer nodes in each layer of the search tree are reserved, and \textit{H-Swarm}'s behavior is same to greed policy. Therefore, the average localization error of BMAVs increases and runtime decreases.}
\label{alpha}
\end{figure}

The AMAV search tree pruning method is able to remove nodes in the search tree which come close in physical space and have similar covariances about BMAVs. 
The most important and computationally demanding operation in pruning is checking $\epsilon$-algebraic redundancy. 
In order to evaluate the relationship between BMAVs' average localization error, $\epsilon$, as well as the corresponding running time, we plot average localization error and runtime against varying $\epsilon$ as Fig. \ref{alpha} shows.
The experimental results show that the time required decreases with the increase of $\epsilon$ because the increase of $\epsilon$ reduces the number of nodes in the search tree. 
However, with the increase of $\epsilon$, the average localization error of BMAVs increases.
This is because the search space decreases and the resulting path of AMAVs is closer to greed policy, and a non-myopic objective cannot be achieved.
In the default setting, the time required for AMAVs planning is less than 500ms, considering the high mobility of AMAVs and the planning module executed every $\delta$, this computational time is trivial. 



% In this section, we first introduce the evaluation setup for experiments in Section \ref{5.1}. Then, the details of the evaluation results and analysis are shown from Section \ref{5.2} to Section \ref{5.8}.
% In the evaluation, we aim to demonstrate the end-to-end performance of our \textit{DeliverSense+}.
% We focus on the following aspects:
% \begin{enumerate}
%     \item We evaluate the performance of our \textit{\textit{DeliverSense+}} system on the scheduling quality, scheduling efficiency, and the total number of routes after scheduling.
%     \item We validate the effectiveness of our system under the impact of different key factors. There are four key factors that significantly influence the algorithm's performance: the number of tasks, the energy capacity, the size of the area of interest, and the utility upper bound.
%     \item We characterize the system computation cost in run time compared with the state-of-the-art algorithms under different system settings. 
%     % Two key impact factors are considered, including the number of DT and the energy budget.
% \end{enumerate}

% \subsection{Evaluation Setup}\label{5.1}
% % Our system is verified by the data collected from a real implemented system. The default number of DT is set as 50, while the default number of each DT's candidate routes is set as 4.
% % The default energy budget is set as 150KJ. 
% Our system is verified by the data collected from real-world delivery service stations.
% The initial energy for each drone is 57,000$KJ$ by default. The delivery weight and other parameters in the energy consumption model are set referring to previous work \cite{dorling2016vehicle}\cite{shan2020looking}.
% Other detailed settings are as follows.

% \subsubsection{Real-world Dataset}
% The real-world dataset comes from the 520 delivery service stations in Shanghai city. The numbers of CDCs and RDCs are 58 and 462, respectively.
% The area of interest to evaluate occupies a size of 80 $km$ $\times$ 80 $km$, part of which is shown in Fig. \ref{dataset}. 
% The default number of sensing tasks is set as 20, and they are generated randomly in the area of interest. 
% The sensing utility weight is uniformly distributed within the range [2,15], while the default sensing utility upper bound is 2000.
% % We generate candidate the delivery routes according to the distribution of the delivery stations. The delivery weight, the energy limitation of each participant, and other parameters in the energy consumption model are set as previous work\cite{xiang2021reusing}.
% % We used 80\% of the generated data for training and the rest 20\% for testing. For the crowdsensing task in the city, we adopt a random function to generate a uniform distribution with 10,000 tasks.
% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
%     \includegraphics[width=0.8\columnwidth]{Figs/map.png}
% \caption{Illustration of the delivery service stations distributed in Shanghai city.}
% \label{dataset}
% %\vspace{-0.8cm}
% \end{figure} 

% \subsubsection{Testbed}
% We evaluate our \textit{DeliverSense+} based on the same hardware configuration, Intel Core i7, 16G memory, RTX2080Ti. All the algorithms are implemented in Python.

% \subsubsection{Metrics}
% To measure the experimental results, we mainly focus on the following four metrics:
% \begin{itemize}
% \item \textit{Scheduling Quality}: Scheduling quality reflects the overall performances of the algorithm on the sensing objective and delivery objective. $\alpha$ is set as 0.5, which means equal importance between the sensing performance and the delivery performance. Therefore, the scheduling quality in the evaluation is calculated as:
% \begin{equation}
%     SQ(V,K) = \max _{\mathbf{x}, \mathbf{t}}\quad 0.5 U'(V,K) - 0.5T'(V,K).
% \end{equation}
% According to Eq. (\ref{ob}), the value of $SQ(V,K)$ lies in $[-0.5,0.5]$.

% \item \textit{Scheduling Efficiency}:
% Scheduling efficiency is defined as the ratio between sensing utility and total energy consumption. 
% It reflects the model's ability to reduce energy consumption and improve the sensing performance simultaneously.
% Considering the limited battery capacity of delivery drones, it is significant to improve the scheduling efficiency $\rho$, which is described as:
% \begin{equation}
%     % \rho = \sum_{k \in \mathcal{K}} \sum_{i, j \in \mathcal{V}} \frac{t_v^k}{c_{ij}x_{ij}^k/s}
%     \rho = \frac{U(V,K)}{E_k}.
% \end{equation}

% \item \textit{Number of Routes}:
% The number of routes is the sum of flight routes required to complete all sensing tasks, which reflects the demand for delivery drone resources.
% % \item \textit{Total Sensing Utility}: 
% % Sensing utility is defined as the product of sensing utility in unit time and the allocated sensing time. In the evaluation, the total sensing utility is calculated with Eq. (\ref{eI}) overall all sensing tasks.

% % \item \textit{Total Delivery Time}:
% % Deliver time is defined as the sum of sensing time and flying time for each delivery. In the evaluation, the total delivery time is calculated according to Eq. (\ref{goal1}) overall delivery drones.

% \item \textit{Run time}: We use the run time of all evaluated algorithms on the same hardware to compare the computation cost. 
% \end{itemize}

% % \textbf{Parameters}:
% % For the coefficient in the Eq. (\ref{goal2}) and objective function (\ref{ob}), we set $\lambda$ =0.5 and $\alpha$=0.5 by default in our implement, respectively. 
% % We adopt ReLU as the activation for all the hidden layers and set the decay coefficient in the loss function as 0.9. In addition, the dropout rate is set to 0.9 for all Transformer blocks.

% \begin{figure*}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
% % \begin{center}
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/overall-Scheduling Quality.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/overall-Scheduling Efficiency.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/overall-Number of Routes.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
% % \end{center}
% \caption{Overall Performance of \textit{DeliverSense+}. (a) Scheduling Quality. (b) Scheduling Efficiency. (c) Number of Routes.}
% \label{overall}
% %\vspace{-0.2cm}
% \end{figure*} 

% % \begin{figure*}[t]
% % % \setlength{\abovecaptionskip}{0.cm}
% % \centering
% %     \includegraphics[width=1.95\columnwidth]{Figs/overall.pdf}
% % \caption{Overall Performance of DeliverSense+. (a) Scheduling Quality. (b) Scheduling Efficiency. (c) Number of Routes.}
% % \label{overall}
% % %\vspace{-0.8cm}
% % \end{figure*} 

% \subsubsection{Baselines Setup}\label{5.2}
% To comprehensively evaluate the performance of \textit{DeliverSense+}, five baselines are implemented for comparison. 
% RC-Ratio is a state-of-the-art approximation algorithm that solves an MINLP problem similar to ours with a theoretical guarantee \cite{wu2020joint}. 
% Therefore, we implement the baselines based on this algorithm and modify some settings to suit our problem.
% For simplicity, our \textit{DeliverSense+} is denoted as \textit{DS} in the evaluation.

% \begin{itemize}
%     \item \textit{RC-Ratio (RC)}: It greedily selects the task node with the largest \textit{RC-ratio} (i.e., the ratio of sensing utility increase to flying distance increase) to construct the travel routes.
%     % \item \textit{Distance greedy (DG)}: It greedily selects the task node with the minimal incremental distance to construct the travel routes.
%     \item \textit{Sensing Utility Greedy (UG)}: It greedily selects the task node with the maximal incremental sensing utility to construct the travel routes.
%     \item \textit{Scheduling Efficiency Greedy (EG)}: It always greedily selects the routes with the maximal scheduling efficiency (i.e., the ratio of sensing utility increase to energy consumption increase) to construct the travel routes.
%     \item \textit{Delivery Time Greedy (TG)}: It greedily selects the task node with the minimal incremental delivery time to construct the travel routes.
%     \item \textit{Random (RA):} It randomly selects the task node to construct the travel routes while satisfying the constraints.
% \end{itemize}

% Note that all the baselines adopt the greedy sensing time allocation strategy and construct the routes with \textit{fast nearest neighbour rule} \cite{rosenkrantz1977analysis}.

% \subsection{Evaluation on the Overall Performance of \textit{DeliverSense+}}\label{5.1}
% % We vary the following settings in order to comprehensively analyze the performance of our system: the number of tasks, the energy capacity of delivery drones, and the sensing utility upper bound. The overall results are shown as follows. 
% % According to the objective function defined in \S\ref{3.1}, the scheduling quality is defined as sensing utility minus delivery time.
% % We compare the overall performance of \textit{DeliverSense+} with various baselines under the default settings in Fig. \ref{overall}. From the comparison, we can make the following observation. 
% In order to illustrate the overall performance of our \textit{DeliverSense+} and five baselines, we plot the results on three metrics under the default settings in Fig. \ref{overall}. From the comparison, we can make the following observations. 

% First, in Fig. \ref{overall}(a), we can find that the average scheduling quality of \textit{DeliverSense+} is 0.153, which shows obvious improvement compared with all baselines.
% Specifically, the average scheduling quality is improved by 46\% and 90\%, compared with RC and TG, respectively. 
% To illustrate the practical meaning of scheduling quality, we take an improvement of 0.01 in scheduling quality as an example. 
% Recall the definition of scheduling quality, which is a weighted sum of the normalized sensing utility and normalized delivery time. 
% Therefore, an improvement of 0.01 in scheduling quality indicates an increase of 800 in sensing utility or a decrease of 224 seconds in delivery time.
% % To illustrate the practical meaning of scheduling quality, we take an improvement of $\delta$ on scheduling quality as an example. 
% % Recall the definition of scheduling quality, which is a weighted sum of the normalized sensing utility and normalized delivery time. 
% % Therefore, the improvement of scheduling quality indicates an increase of $80000\delta$ in sensing utility or a decrease of $22,400\delta$ seconds in delivery time.
% % Therefore, the improvement of scheduling quality indicates an increase in sensing utility or a decrease in delivery time.
% % Since the default value of $\alpha$ is 0.5 in the experiment, the improvement $\delta$ is equivalent to the improvement of the normalized sensing utility of $80000\delta$. 
% % From the perspective of delivery performance, the improvement $\delta$ means that around $22,400\delta$ seconds can be saved for delivery within each schedule.   
% This validates our idea that combining the strength of DRL and heuristic can help gather more sensing information while spending less extra delivery time. The improvement comes from our algorithm's ability to assign sensing tasks for delivery drones and plan flight routes from a holistic perspective.

% Second, for the average scheduling efficiency, \textit{DeliverSense+} significantly obtains the best overall performance, as shown in Fig. \ref{overall}(b). Specifically, \textit{DeliverSense+} improves the scheduling efficiency by 30\%, 64\%, 39\%, 59\%, and 101\%, over RC, UG, EG, TG, and RA, respectively. This shows that \textit{DeliverSense+} has learned the ability to balance energy consumption and sensing utility, which attributes to the integration of reinforcement learning and heuristic method.

% Finally, from Fig. \ref{overall}(c), we discovered an interesting phenomenon that \textit{DeliverSense+} maintains about 5 routes on average after scheduling, while RC and EG methods require about 12 and 15 routes, respectively. 
% In other words, \textit{DeliverSense+} is able to achieve better performance with fewer delivery drones, compared with the baselines that have the most similar performance. 
% This indicates that \textit{DeliverSense+} is able to select a less number of delivery drones to derive high scheduling quality, which reduces the total energy consumption and contributes to the improvement of scheduling efficiency in Fig. \ref{overall}(b).


% % The comparisons with the five baselines show that we can significantly improve both the sensing profit and the delivery profit under all experiment settings by incorporating reinforcement learning and greed algorithm.
% % The comparison of the run time also shows that our \textit{DeliverSense+} is more efficient than the state-of-the-art algorithm when the problem scale increases.

% % Besides, the TimeAllocator model are proved to be comparable with the state-of-the-art algorithms RT \cite{xiang2021reusing}.
% \begin{figure*}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
% % \begin{center}
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/task-Scheduling Quality.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/task-Scheduling Efficiency.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/task-Number of Routes.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
% \caption{Performance evaluations of \textit{DeliverSense+} in terms of the number of tasks on three metrics. (a) Impact of the number of tasks on scheduling quality. (b) Impact of the number of tasks on scheduling efficiency. (c) Impact of the number of tasks on the number of routes. }
% \label{taskimpact}
% %\vspace{-0.2cm}
% \end{figure*} 

% \begin{figure*}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
% % \begin{center}
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/Energy-Scheduling Quality.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/Energy-Scheduling Efficiency.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/Energy-Number of Routes.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
% % \end{center}
% \caption{Performance evaluations of \textit{DeliverSense+} in terms of energy capacity on three metrics. (a) Impact of energy capacity on scheduling quality. (b) Impact of energy capacity on scheduling efficiency. (c) Impact of energy capacity on the number of routes. }
% \label{energyimpact}
% %\vspace{-0.2cm}
% \end{figure*} 





% \subsection{Effect the Number of Tasks}\label{5.2}
% We show the impact of the number of tasks on scheduling quality, scheduling efficiency, and route number in Fig. \ref{taskimpact}.
% We changed the number of tasks from 15 to 40 with a step size of 5, while we leave other parameters unchanged with their default values.
% From the comparison, we can make the following observations.

% From Fig. \ref{taskimpact}(a), we can see that \textit{DeliverSense+} consistently outperforms all five baselines in terms of scheduling quality. For example, when the number of tasks is 40, \textit{DeliverSense+} achieves a scheduling quality of 0.10, compared to RC given the best line, with a 37\% improvement. 
% Besides, for all approaches, the scheduling quality improves as the number of tasks increases. This is because the delivery drones are able to perform more sensing tasks, which increases their total sensing utility. Increasing the number of sensing tasks indicates a larger search space for scheduling the delivery routes, and selecting the tasks with manually designed rules for each delivery route tends to significantly increase the delivery time. 
% Therefore, the baselines fail to balance the trade-off between delivery time and sensing utility. 
% In contrast, the incorporation of the DRL successfully guides our algorithm to assign an adequate number of sensing tasks for each delivery drone, which helps the algorithm to obtain more sensing utility in scheduling.
% % On average, for scheduling quality, \textit{DeliverSense+} significantly improves 35\%, 58\%, 48\%, 79\%, and 32\% over RC, UG, EG, TG and RA approach, respectively.
% % leverages neural networks to fast approximate the optimum, thus handle the large-scale problem successfully.  
% % This is because the more sensing tasks allows not only more sensing time allocation, but also more sensing tasks could be assigned to the delivery drones, which leads to higher sensing profit. 

% % within the number of tasks range of 150KJ to 200KJ, the total profit, the sensing time profit, and the delivery profit increases monotonically, as shown in Fig. \ref{energy impact}(c) and Fig. \ref{energy impact}(d).
% % But the impact of the energy budget decreases as it gets larger, mainly because the delivery profit has converged. For example, from Fig. \ref{energy impact}(d), we can see some slight declines in the delivery profit with an increasing energy budget. 
% % \item 
% The effects of task number on scheduling efficiency are also investigated as shown in Fig. \ref{taskimpact}(b). 
% While the scheduling efficiency of \textit{DeliverSense+} keeps improving with the increase of sensing tasks, this metric of other baselines decreases instead. Recall the definition of scheduling efficiency, which is the ratio of sensing utility and energy consumption. Since UG and TG focus more on a single metric, their performance on scheduling efficiency is not satisfactory enough. 
% RC and EG perform slightly better than other baselines, because they consider more indicators when deciding the search direction.
% Without effectively modeling the cooperation between different routes, these baselines schedule the delivery drones with a considerable increase in flying time, which lead to large energy consumption. When the increase in delivery time is greater than the improvement of sensing utility, the scheduling efficiency decreases significantly.
% It is noticed that our \textit{DeliverSense+} outperforms all baselines with variant numbers of tasks, which shows the obvious advantage of our design.

% To illustrate the effect of task number on the demand for delivery drones, we demonstrate the change in the number of routes in Fig. \ref{taskimpact}(c). TG, EG, and RC grow as the task number increases, but \textit{DeliverSense+} does not increase apparently. This indicates that even though the growth of task numbers complicates the optimization problem, our \textit{DeliverSense+} is still able to keep a high scheduling efficiency and scheduling quality with a small number of delivery drones. This shows the robustness of our \textit{DeliverSense+} under uncertainty in the number of tasks. 
% % For DeliverSense+, the iterative optimization scheme helps it capture the dependency of the variables in the problem, thus it maintains a better performance when the number of sensing tasks increases.
% % This is because TG and RG focus more on a single metric rather than the overall performance. However, the scheduling efficiency is calculated based on both sensing utility and energy consumption, which is related to the hovering time and flying time. 
% % However, the sensing tasks are randomly distributed in the area of interest and the selected number of tasks increases with the energy budget grows. Thus the \textit{DeliverSense+} tends to choose the sensing tasks with larger sensing benefits while sacrificing the coverage performance, to obtain a better total sensing profit.




% \begin{figure*}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
% % \begin{center}
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/dis-Scheduling Quality.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/dis-Scheduling Efficiency.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/dis-Number of Routes.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
% % \end{center}
% \caption{Performance evaluations of \textit{DeliverSense+} in terms of the area size on three metrics. (a) Impact of the area size on scheduling quality. (b) Impact of the area size on scheduling efficiency. (c) Impact of the area size on the number of routes. }
% \label{areaimpact}
% %\vspace{-0.2cm}
% \end{figure*} 

% \subsection{Effect of the Energy Capacity}\label{5.5}
% Fig. \ref{energyimpact} shows the impact of the energy capacity for delivery drones. We vary the energy capacity from 40,000 $KJ$ to 75,000 $KJ$ with a step of 5,000 $KJ$. From Fig. \ref{energyimpact}(a)-(c), we can make the following observations.

% Fig. \ref{energyimpact}(a) illustrates that \textit{DeliverSense+} outperforms all five baselines in terms of scheduling quality. 
% For example, \textit{DeliverSense+} reaches a scheduling quality of 0.21 when the energy capacity is 75,000 $KJ$, beating the best baseline EG by 24\%, whose scheduling quality is just 0.16. On average, \textit{DeliverSense+} outperforms RC, UG, EG, TG, and RA methods by 17\%, 270\%, 18\%, 127\%, and 692\% in terms of scheduling quality, respectively. Besides, a large energy capacity leads to high scheduling quality for most of the methods at the beginning, but when the energy capacity reaches more than 70,000 $KJ$, we discover that the impact on scheduling quality gradually diminishes. This may be explained by the fact that with the growth of energy capacity, the delivery drones have more remaining energy to hover and collect sensing data. However, when the energy capacity exceeds a threshold, all the sensing tasks are completed (i.e., the task utilities reach their upper bound), thus the scheduling quality does not rise anymore.

% From Fig. \ref{energyimpact}(b), we see that the scheduling efficiency of \textit{DeliverSense+} increases monotonically as the energy capacity grows. \textit{DeliverSense+} shows consistent advantage of scheduling efficiency with variant energy capacities of delivery drones. Especially, \textit{DeliverSense+} achieves up to a scheduling efficiency of 0.12 when the energy capacity is $55,000KJ$, which is 29\% higher than the best baseline RC.
% Meanwhile, it is also worth noting that the route number of \textit{DeliverSense+} declines gradually, as shown in Fig. \ref{energyimpact}(c). This is because a larger energy capacity allows a delivery drone to conduct more sensing tasks in a flight. As a result, a small group of delivery drones can complete all the tasks with less total flying distance, which in turn rise the scheduling efficiency. It implies that the energy capacity will become a limiting factor when there are only a few delivery drones can be scheduled.
% The comparison also indicates that \textit{DeliverSense+} captures the general structure of this NP-hard combinatorial optimization problem, thus it consistently assigns the most appropriate number of drones to perform the task. 

% \begin{figure*}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
% % \begin{center}
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/uB-Scheduling Quality.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/uB-Scheduling Efficiency.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.6\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/uB-Number of Routes.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
% % \end{center}
% \caption{Performance evaluations of \textit{DeliverSense+} in terms of the sensing utility upper bound on three metrics. (a) Impact of the sensing utility upper bound on scheduling quality. (b) Impact of the sensing utility upper bound on scheduling efficiency. (c) Impact of the sensing utility upper bound on the number of routes. }
% \label{ubimpact}
% %\vspace{-0.2cm}
% \end{figure*} 
% \subsection{Effect of the Area Size}\label{5.6}
% Next, we show the impact of area size in Fig. \ref{areaimpact}. We consider the situations that the service stations occupy a size of area from $2.7 km \times 2.7km$ to $3.3 km \times 3.3km$. The primary observations are summarized as follows.

% Fig. \ref{areaimpact}(a) reveals how the area size affects the scheduling quality of different methods. First, From Fig. \ref{areaimpact}(a), we can observe that \textit{DeliverSense+} exceeds the performance of all competing baselines in the terms of scheduling quality. Especially, when the area size is $2.7 km \times 2.7km$, \textit{DeliverSense+} reaches the best scheduling quality. 
% % On average, DeliverSense+ outperforms RT, RA, CG, DG, and PG methods by 42\%, 25\%, 31\%, 38\%, and 37\% in terms of scheduling quality, respectively.
% Second, it is noticed that all methods show a decline in scheduling quality with the growth of area size. The reason behind this phenomenon is that the larger area will lead to a longer flying distance, which indicates the delivery time increase. However, even in these cases, \textit{DeliverSense+} outperforms all the baseline approaches by more than 14\% percent in terms of scheduling quality. 
% Since the sensing tasks are assigned to several delivery drones, a larger area size implies a smaller number of tasks in the unit area on average. Therefore, to improve the scheduling efficiency, it is significant to determine the number of tasks to execute with the consideration of the area size.
% % This means that our method successfully learned an effective policy to assign the sensing tasks, 

% Fig. \ref{areaimpact}(b) depicts the scheduling efficiency of all methods when varying the area size. The scheduling efficiency trend of all methods is similar to the scheduling quality in Fig. \ref{areaimpact}(a). This is due to the same reason mentioned in the previous paragraph. Furthermore, the average route number of \textit{DeliverSense+} shows little fluctuation with variant area size, as shown in Fig. \ref{areaimpact}(c). This indicates that the increase in area size would not apparently influence the task assignment strategy of our \textit{DeliverSense+}. Indeed, the key factor that influences the overall performance in this scenario is the route planning strategy. Therefore, by utilizing the coordination between the delivery drones to optimize the routing scheme, \textit{DeliverSense+} beats the best baseline RC in terms of both scheduling quality and scheduling efficiency.
% This comparison result again validates the effectiveness of the combination of DRL and heuristic method.
% % In addition, DeliverSense+ always has the best performance when the area size grows, which validates the effectiveness of the our combination of DRL and heuristic methods. 


% \subsection{Effect of the Task Utility Upper Bound}\label{5.4}
% We present the impact of the sensing utility upper bound in Fig. \ref{ubimpact}. The sensing utility upper bound is changed from 1,700 to 2,300. We can make the following observations from the experimental results.

% The effects of sensing utility upper bound on scheduling quality are investigated as shown in Fig. \ref{ubimpact}(a). First, comparing the scheduling quality of different methods, we see that \textit{DeliverSense+} consistently shows better performance than baselines. This proves that our algorithm effectively allocates reasonable sensing time for the tasks that bring higher sensing utility. Second, with a higher sensing utility upper bound, the scheduling quality of all methods increases. This is because the increase in sensing utility upper bound allows the drones to allocate more sensing time to collect sensor data, which results in total sensing utility improvement.
% % Fig \ref{ubimpact}(a) depicts that DeliverSense+ outperforms all other baselines in terms of scheduling quality for any sensing utility upper bound. For example, when the sensing utility upper bound is 2000, DeliverSense+ achieves a scheduling quality of xxx, compared to 46,375 given by the best baseline RC. 
% % On average, for the scheduling quality, \textit{DeliverSense+} significantly improves 42\%, 25\%, 31\%, 38\%, 37\% over RT, RA, CG, DG, and PG approach, respectively.

% Fig. \ref{ubimpact}(b) displays that the scheduling efficiency of \textit{DeliverSense+} and baselines rise with the increase in sensing utility upper bound. Each delivery drone aims to collect as much data as possible when the constraints remain satisfied. As a result, the total sensing utility rises and the scheduling efficiency naturally rises.
% We can see that \textit{DeliverSense+} always has the highest scheduling efficiency while comparing different sensing utility upper bound. For example, when the sensing utility upper bound is 2000, \textit{DeliverSense+}'s scheduling efficiency is 0.12, which is 29.7\% and 39.4\% higher than RC and EG, respectively. The reason behind this trend may be that \textit{DeliverSense+} captures the relationship between sensing utility and energy consumption, thus it can complete tasks with less energy consumption.
% In addition, from Fig. \ref{ubimpact}(c), we can see the total route numbers of all methods are not sensitive to the sensing utility upper bound. This implies that compared to other methods our \textit{DeliverSense+} is more attractive to delivery companies, since it can achieve higher scheduling quality with much fewer delivery drones.
% % DeliverSense+ maintains about 7 routes for any sensing utility upper bound, while RC and EG methods require about 12 and 15 routes, respectively. In other words, DeliverSense+ is able to achieve better performance with fewer delivery drones, compared with the baselines that have the most similar performance. This is caused by the fact that DeliverSense+ learns a reasonable policy for task assignment, and then a small number of delivery drones are able to cover all the sensing tasks without large energy consumption.


% % while the total profit of \textit{DeliverSense+} decreases slightly with more than 80 DTs. 
% % This is because the difficulty of getting the optimal solution is directly related to the problem's scale, i.e., the larger number of DTs will lead to a more complex searching space of the problem with more coupled variables. 
% % However, even in these cases, the \textit{DeliverSense+} outperforms all the baseline approaches by more than 25 percent. 
% % In addition, The decreases in the total profits are mainly due to the degrades of the delivery profit, while there is still a slight increase in the sensing time profit.

% % When the number of DTs is 100, the five baseline approaches achieve similar results in terms of the total profit with a value less than 45,000, while the \textit{DeliverSense+} maintains a total profit of more than 45,000. This is because the reinforcement learning scheme benefits the learning process of \textit{DeliverSense+}. Without capturing the general structure of this NP-hard combinatorial problem, even the state-of-the-art method RT cannot maintain a good performance. 
% % For example, as shown in Fig. \ref{DT impact}(d), when the number of DTs range from 70 to 100, RT has the worst performance in terms of the delivery profit among all five baselines. The comparison indicates that RT algorithm may fail to approximate the optimal solution and the performance degrades rapidly. On the contrary, though our \textit{DeliverSense+} shows a slight decrease, it consistently shows significant advantages over baselines.

% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
% % \begin{center}
%     \subfigure[]{
%         \begin{minipage}[t]{0.48\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/alpha-Weighted Objectives.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
%     \subfigure[]{
%         \begin{minipage}[t]{0.48\columnwidth}
%             \centering
%             \includegraphics[width=1\columnwidth]{Figs/alpha-Scheduling Efficiency.png}
%             %\caption{fig1}
%         \end{minipage}%
%     }%
% % \end{center}
% \caption{Performance evaluations of \textit{DeliverSense+} in terms of $\alpha$. (a) Impact of $\alpha$ on delivery time and sensing utility. (b) Impact of $\alpha$ on scheduling efficiency.}
% \label{alphaimpact}
% %\vspace{-0.2cm}
% \end{figure} 

% \subsection{Impact of coefficients in the objective function}\label{5.7}
% In order to check how the model coefficient $\alpha$ in Eq. (\ref{ob}) affect the performance, we plot $\alpha$ with variant values in Fig. \ref{alphaimpact}. The value $\alpha$ is set from 0 to 1 with a step of 0.1. Note that since $\alpha$ indicates the trade-off between the sensing performance and delivery performance, it could be adjusted according to the practical requirements.
% As shown in Fig. \ref{alphaimpact}(a), the weighted sensing utility consistently increases with the increase of the $\alpha$ value, while the weighted delivery time keeps decreasing. This is because that larger $\alpha$ value biases the model to focus more on the sensing utility, thereby the penalty for delivery time decreases.
% Meanwhile, we discovered an interesting phenomenon in Fig. \ref{alphaimpact}(b) that as the $\alpha$ value rises from 0.5 to 1, the scheduling efficiency begins to degrade.
% This implies that a suitable model coefficient of \textit{DeliverSense+} will contribute to the overall performance. When we assign equal importance to the dual objectives, the scheduling efficiency is more close to the optimum. 
% In summary, the evaluation result shows that \textit{DeliverSense+} could respond correctly to the parameter settings in the objective function.

% \subsection{Computational Efficiency}\label{5.8}
% To evaluate the computation efficiency and advantages of adopting the reinforcement learning algorithm, we compare the average run time for a scheduling decision process in Fig. \ref{runtime}. We mainly focus on the run time under different numbers of tasks, because the combination choices of decision variables grow exponentially with the number of tasks grows, which incurs a significant increase in computational complexity. Other parameters are set by default.
% We can see that when the number of tasks is less than 30, all baselines have a stable performance in terms of run time. However, as the number of tasks increases, the run time of EG and RC increases dramatically. Especially, when the task number is 60, the run time of EG reaches about 100 seconds, which is nearly 100 times longer than \textit{DeliverSense+} on average.
% The reason behind is that both EG and RC rely on the \textit{fast nearest neighbour rule} \cite{rosenkrantz1977analysis} to construct flight routes, and the computation complexity can be expressed as $\mathcal{O}(\mathcal{R} \cdot r(n)^2)$, where $\mathcal{R}$ is the number of routes and $r(n)$ is the number of tasks on route $r$, respectively. On the contrary, the computation complexity of constructing routes in \textit{DeliverSense+} is $\mathcal{O}(T)$, where $T$ is the maximal number of rewriting steps. 
% % and $|\mathcal{N}|$ is the total number of sensing tasks, respectively.
% % Overall, the run time can be improved by about xx\%, xx\% on average via \textit{DeliverSense+} compared with EG and RC, respectively.
% Overall, \textit{DeliverSense+} shows advantages in run time over all baselines when dealing with a large-scale problem.
% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{0.cm}
% \centering
%     \includegraphics[width=0.8\columnwidth]{Figs/task-Runtime (s).png}
% \caption{Approximate run time of \textit{DeliverSense+} and baselines.}
% \label{runtime}
% %\vspace{-0.8cm}
% \end{figure} 
% % The number of DTs is tuned from 50 to 100, while the energy budget is set from 150KJ to 200KJ.
% % Note that the other baselines CG, DG, and PG are based on the greedy principle, which only needs to sort the items in $\mathcal{O}(n)$ computational complexity. Similarly, the baseline RA randomly selects several routes and allocates the sensing time according to the greedy algorithm with ignorable computation. 
% % Therefore we aim to compare the run time with the state-of-the-art algorithm RT which has the performance most similar to our \textit{DeliverSense+} instead of the heuristic baselines approaches. 
% % From Fig. \ref{runtime}, we can see that although the run time of EG and RC grow exponentially with the number of tasks. Specially, when the number of tasks is up to 40, the run time of EG is more than xxxs, 

% % Besides, as shown in Fig. \ref{runtime}(b), when the energy budget is less than 170 KJ, both \textit{DeliverSense+} and RT have a stable performance in terms of run time with less than 200 seconds. However, when the energy budget is more than 170 KJ, the RT algorithm run time increases significantly, which is nearly 3 times longer than \textit{DeliverSense+} on average. For example, when the energy budget is 200KJ, the run time of RT is around 1,000 seconds. On the contrary, the run time of \textit{DeliverSense+} is only about 200 seconds. Overall, the run time can be improved by about 64\% on average via \textit{DeliverSense+} compared with RT.





% % In addition, with the increase of $\lambda$, the sensing time profit increases monotonically and the sensing coverage profit degrades instead. 
% % Suitable parameters of \textit{DeliverSense+} will contribute to the overall performance.
% % Specifically, Fig. \ref{coef impact}(a) and Fig. \ref{coef impact}(b) indicate the trade-off of the sensing profit and the delivery profit, which could be adjusted according to the practical requirements. 
% % The evaluation result shows that \textit{DeliverSense+} could respond correctly to the parameter settings in the objective function.



% % We also evaluate the run time of \textit{DeliverSense+} in different numbers of selected routes, as illustrated in Fig. \ref{select impact} (d). When the number of selected routes is greater than 10, \textit{DeliverSense+} spends more than 150 seconds on average for one solution, 
% % The combinations choices of these variables grow exponentially with the number of high-coupled variables, thus incurring a higher computational complexity.
% % Note that When the number of selected routes is more than 13, the run time begins to decrease instead. 
% % This is because, under the current energy budget setting, the energy budget is used up when the number of routes is greater than a threshold. Therefore the algorithm does not need to spend effort allocating the sensing time.

% % \end{itemize}





==> intro.tex <==
\vspace{-0.4em}
\section{Introduction}

Drone swarms, especially Micro Aerial Vehicles (MAV) swarms, offer transformative potential in diverse fields such as industry \cite{wang2019dynamic}, agriculture \cite{khochare2021heuristic}, urban computing \cite{zhao2022dronesense}, and emergency response \cite{rashid2020socialdrone}, leveraging their inherent advantages of working scalability \cite{bertizzolo2020swarmcontrol}, flexibility \cite{wang2021lifesaving}, adaptability \cite{li2021physical}, \etc.
There are forecasts that the market size for MAV swarm-supported applications will reach \$ 279 billion by 2032 \cite{Global-Drones}.

A MAV swarm typically consists of: 
$(i)$ a handful of advanced MAVs (AMAVs) that are computationally intensive yet expensive \cite{shen2022joint};
and $(ii)$ a larger group of resource-limited and cost-effective basic MAVs (BMAVs) \cite{wang2022h}.
The former primarily handles data management, communication, and high-level computation tasks, while the latter concentrates on environmental exploration and video capturing \cite{li2022intelligent}. 
The AMAV-BMAV collaboration paradigm achieves an optimal balance between the swarm's sensing capabilities and cost, facilitating its widespread adoption by extensive applications including Amazon disaster relief \cite{rashid2020computational}, DJI industrial inspection \cite{yang2019intelli}, and aerial imaging \cite{trotta2018uavs}, \etc.

\begin{figure}[t]
    \centering
        \includegraphics[width=0.95\columnwidth]{Figs/intro.png}
    \vspace{-0.3cm}
     \caption{Introduction of heterogeneous MAV swarm.}
    \label{intro}
    \vspace{-0.6cm}
\end{figure} 

Accurate and real-time localization is a crucial component of MAV swarms \cite{shan2021ultra}. 
Specifically, each MAV is required to determine its own real-time location for flight control \cite{chi2022wi}, obstacle avoidance \cite{xu2020edge}, \etc. 
Current localization practice can be divided into two categories:

% \textcolor{red}{its own real-time 6-degree-of-freedom (6-DoF) pose (\ie, 3-DoF location plus 3-DoF orientation)}

\noindent $\bullet$ \textbf{Extra-infrastructure based solutions}, where external specific devices provide reference signals (\eg, GPS \cite{sharp2022authentication}, RTK \cite{wang2022micnest}, radio \cite{li2021infocom_itoloc}, or acoustic \cite{wang2022micnest}) for localization.
However, they often face limitations in accuracy.
% \textcolor{red}{, (\ie, typically with biases $>0.5m$)} and may not provide orientation information. 
Moreover, these solutions are heavily reliant on the pre-deployment of expensive localization infrastructure. 
In scenarios such as disaster relief in the wild, the infrastructure absence or destruction can lead to localization failures \cite{chen2015drunkwalk}.

\noindent $\bullet$ \textbf{Intra-onboard-sensor based solutions.}
These solutions leverage onboard sensors like cameras, IMU, and LiDAR, along with SLAM techniques, to achieve high-precision pose estimation\cite{dong2019infocom_pairnavi, xu2022swarmmap}. 
However, they fail to consider different MAVs' varying perception and computational resources.
Specifically, while AMAVs can effectively utilize these solutions, BMAVs cannot afford expensive high-precision sensors, leading to accuracy bottlenecks. 
% (\eg, high-resolution camera, high-beam LiDAR, high-end IMU), 
Furthermore, BMAVs' limited computational results in significant computation delays and accumulated errors as illustrated in Fig.\ref{intro} \cite{xu2020edge} $\footnote{ AMAV is equipped with Intel(R) i7-8750H and 32G RAM, BMAV is equipped with Cortex-A53 and 1G RAM. Results in Fig.1 and Fig.2a are measured with MH\_02 of EuRoC dataset\cite{burri2016euroc} and CCM-SLAM \cite{schmuck2019ccm}}$. 
% Additionally, AMAVs enjoy the responsibility of computing their relative pose in relation to the surrounding MAVs\tocite.

\noindent \textbf{Remark:} In summary, there still lacks a low-cost, high-precision, and real-time localization solution for MAV swarms, especially for those lightweight BMAVs.


% In this work, we aim to enhance the localization accuracy and real-time performance of BMAVs while reducing their reliance on: $(i)$ high-end sensors;
% $(ii)$ intensive computational resources;
% and $(iii)$ pre-deployed localization infrastructures.
\noindent \textbf{The primary goal of this work} is to improve BMAVs' localization accuracy and efficiency while minimizing their dependence on high-end sensors, intensive computational resources, and pre-deployed localization infrastructures. 
Our key insight is to upgrade AMAVs as \textit{mobile localization infrastructures} for BMAVs. 
Specifically, AMAVs can utilize computer vision techniques to track BMAVs' poses from a global perspective \cite{wang2016apriltag}, generate external observation equations for BMAV's pose estimation \cite{xu2021mobisys_followupar}, and eventually minimize the cumulative errors.
% and then using the results to correct BMAVs' poses, reducing cumulative errors.
% With their global perspective and computational capabilities, AMAVs can track, observe, and correct BMAVs' poses, reducing cumulative errors. 
Additionally, BMAVs can offload the complex pose optimization tasks to AMAVs, enhancing their real-time performance. 
By transforming AMAVs into moving localization beacons, we aim to create a dynamic, scalable, and cost-effective localization system suitable for large-scale heterogeneous MAV swarms.

However, turning this insight into a practical system is non-trivial.
Two grand challenges ought to be solved:

\noindent \textbf{$\bullet$ Pose optimization with BMAV's noisy estimation.}
BMAVs have limited computational resources and are mainly equipped with cameras and high-noise motion sensors (\eg, IMU), leading to sparse point cloud generation, and a trade-off between latency and motion-tracking accuracy, which complicates the pose optimization with AMAV's observations (Fig. \ref{motivation}a). 
Existing multi-device joint pose calibration methods, based on visual-inertial fusion, assume an identical distribution of pose estimation errors across devices \cite{dong2019infocom_pairnavi}, which doesn't cater to BMAVs' higher localization noise. 
Other methods ideally assume observations from AMAVs include BMAVs locations that are linear to the actual locations, disregarding the non-linear nature of observations \cite{wang2022h}.
% with added Gaussian noise
% Existing multi-device joint pose calibration methods, based on visual-inertial fusion, assume either a uniform point cloud density or an identical distribution of pose estimation errors across devices \cite{dong2019infocom_pairnavi}, which doesn't cater to BMAVs' higher localization noise.


\noindent \textbf{$\bullet$ Resource allocation with AMAV's dynamic coverage.}
Given the limited field of view (FoV) of an individual AMAV, it's crucial to determine which BMAVs it should serve and allocate resources accordingly for localization services \cite{shi2020drone}. 
However, as both AMAVs and BMAVs are in constant motion, the observable BMAVs by each AMAV keep changing, necessitating dynamic adjustment of resource allocation strategies. 
Moreover, the localization effectiveness is also influenced by the distance and bearing angle changes between AMAVs and BMAVs, complicating the optimal dynamic resource allocation strategy formulation (Fig. \ref{motivation}b).

\begin{figure}[t]
\setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
\setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
\setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
\centering
    \subfigure[Accuracy vs. latency]{
        \centering
            \includegraphics[width=0.43\columnwidth]{evaFigs/runtimex.png}
            % \includegraphics[width=0.43\columnwidth]{evaFigs/runtime.png} % 图
    }
    \subfigure[Accuracy of visual sensor]{
        \centering
            \includegraphics[width=0.5\columnwidth]{evaFigs/measure_error.png}
    }
\caption{Motivating example.}
% In Fig. (b), scenario 1 is a short distance (0.6m) and small bearing angle (0°), scenario 2 is a short distance and large bearing angle (30°), scenario 3 is a long distance (1.5m) and small bearing angle, and scenario 4 is a long distance and large bearing angle.
\label{motivation}
\vspace{-0.6cm}
\end{figure}

To tackle the above challenges, we design and implement H-Swarm, 
a new framework that transforms AMAVs into mobile localization infrastructures, specifically designed for low-cost and resource-constrained BMAVs. 
The primary goal of H-Swarm is to provide accurate and real-time localization performance. 
By implementing H-Swarm, MAV swarm systems can reduce their reliance on additional localization infrastructures and high-end onboard sensors, thereby facilitating the widespread deployment of swarm technology.




% Micro Aerial Vehicles (MAV) swarms are widely utilized in disaster response and environmental monitoring. Their autonomous exploration offers valuable environmental information due to the following advantages:
% (1) High Mobility: MAVs possess the capability to access areas that are challenging or impossible for humans to reach;
% (2) Widespread deployment: Compared to traditional manned aircraft, MAVs have lower operational and maintenance costs. This affordability enables their efficient and widespread deployment, facilitating rapid response efforts.

% Typically, the MAV swarm is composed of two distinct types of MAVs with heterogeneous resources:
% (1) Advanced MAVs (AMAVs) - a small number of resource-intensive MAVs possess premium sensing and computing capability. AMAVs can carry heavier and more sophisticated sensor equipment, have greater endurance, and can be used for tasks such as communication relays.
% (2) Basic MAVs (BMAVs) - a significant number of resource-constrained MAVs, responsible for navigating toward destinations for the purpose of sensing. BMAVs have lower costs and are lightweight, making them suitable for widespread deployment and collaborative work. 

% The key components for effectively employing a MAVs swarm are localization and navigation, which means each MAV needs to obtain its own location information in real-time, as highlighted in recent studies \cite{famili2022pilot, wang2022micnest, ruiz2016demo}. 
% Researchers propose various approaches to maintain MAV swarm localization accuracy during navigation, including: 
% (1) relying on external infrastructures, such as GPS, radio, and motion capture devices to provide reference signals for localization \cite{chen2020distributed, chi2022wi, preiss2017crazyswarm}. These devices can be used outdoors or in a laboratory environment \cite{chi2022wi}. However, the localization accuracy of these methods is low, and the existing infrastructure may be damaged or destroyed in a disaster. Furthermore, it may not be possible to manually install supporting sensors such as beacons in advance.
% (2) relying on onboard sensors utilize cameras, IMUs, LiDAR, and employ SLAM (Simultaneous Localization and Mapping) techniques to achieve high-precision localization. However, these solutions overlook the heterogeneity of perception and computational resources among devices. While AMAVs can handle such solutions, BMAVs, on the one hand, cannot carry expensive high-precision sensors, resulting in limited accuracy. On the other hand, there are significant computation delays and accumulated errors in BMAVs due to limited computational capabilities.
% In a nutshell, none of the previous solutions can achieve a low-cost, high-precision, and real-time localization system suitable for large-scale heterogeneous MAV swarm.


% \begin{table}[]
% \centering
% \caption{The cost of the AMAV and the BMAV.}
% \begin{threeparttable}
% \begin{tabular}{cccccc}
% \hline
% \multicolumn{6}{c}{Cost of AMAV and BMAV (\$)}                                                                                        \\ \hline
% \multicolumn{1}{c|}{Type} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Auto-\\ pilot\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Embedded\\ computer\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Optical\\ Flow\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Tracking \\ camera\end{tabular}} & All  \\ \hline

% \multicolumn{1}{c|}{AMAV\tnote{*}} & \multicolumn{1}{c|}{400}                                                   & \multicolumn{1}{c|}{800}                                                          & \multicolumn{1}{c|}{/}                                       & \multicolumn{1}{c|}{324}                                                        & 1524 \\ \hline
% \multicolumn{1}{c|}{BMAV\tnote{**}} & \multicolumn{1}{c|}{200}                                                   & \multicolumn{1}{c|}{/}                                             & \multicolumn{1}{c|}{50}                                                     & \multicolumn{1}{c|}{/}                                           & 250  \\ \hline
% \end{tabular}

% \begin{tablenotes}
%     \footnotesize
%     \item[*] The AMAV consists of Pixhawk 4 autopilot, Nvidia Jetson Xavier NX embedded computer, Intel realsense T265 tracking camera. All data are from https://www.amazon.com.
%     \item[**] The BMAV is based on Bitcraze Crazyflie nano quadcopter, and the data are from https://store.bitcraze.io/.
% \end{tablenotes}
% \end{threeparttable}
% \label{cost}
% \vspace{-2.0em}
% \end{table}

% In this paper, we have the following insight: by fully utilizing the sensing capabilities of heterogeneous MAV swarm, we can leverage AMAVs as external mobile localization infrastructure for BMAVs, building upon the localization based on onboard sensors of BMAVs.
% This approach aims to enhance the localization accuracy and real-time performance of BMAVs while reducing their reliance on high-precision sensors and intensive computational resources. As a result, it not only lowers the overall swarm cost but also expands the deployment range.
% Albeit inspiring, translating this intuition into a practical AR framework is non-trivial and faces significant challenges:
% \begin{itemize}
%     \item \textbf{The BMAVs' accurate localization with limited capability.} BMAVs have limited computing capability and are equipped with basic localization sensors such as IMU (Inertial Measurement Unit) and optical flow sensors. Their localization error tends to increase over time due to noisy measurements using conventional methods \cite{borenstein1996navigating}. There is a lack of a method to address the localization of BMAVs under constrained estimation, which leads to precision bottlenecks in their localization. 
%     \item \textbf{The limited sensing resource allocation of AMAV for BMAVs.} Different BMAVs and AMAVs have varying locations and localization errors, making AMAV sensing resource allocation complex for dynamic coverage. Furthermore, the distance between AMAVs and BMAVs affects observation quality, requiring a quantity-quality trade-off. Additionally, restricted AMAV velocity causes BMAV displacement during observations, adding to the computational cost \cite{kunze2018artificial}.
% \end{itemize}


% To tackle the above challenges, we design and implement H-Swarm, the first framework that upgrades the localization paradigm for coordinated localization of heterogeneous MAV swarm, enabling the full utilization of resources in AMAVs as an external mobile localization infrastructure for BMAVs. This has resulted in a scalable, low-cost, high-precision, real-time localization solution suitable for heterogeneous MAV swarms.
% H-Swarm can be integrated into the existing MAV swarm localization framework, which further expands the scale of the MAV swarm and improves the localization accuracy of the MAV swarm.

In H-Swarm, we first verify and model the localization error of BMAVs through experimental methods. Building upon this, we design an \textit{error-tolerant joint pose estimation} model
% \textit{ETJE}, an \textbf{E}rror-\textbf{T}olerant \textbf{J}oint \textbf{E}stimation model, 
% to integrate constrained estimation from BMAVs with discontinuous observations from AMAVs to perform joint estimation of BMAVs' location.
to integrate constrained estimation which has growing error from BMAVs with discontinuous observations from AMAVs to perform joint estimation of BMAVs' location.
Secondly, to allocate the sensing resource of AMAV for dynamic coverage, we design a \textit{graph-based adaptive grouping-scheduling} strategy. 
% This strategy dynamically groups the AMAVs and BMAVs based on the Voronoi diagram to conserve AMAV's sensing resources at first. 
This strategy dynamically groups the AMAVs and BMAVs to conserve the sensing resources of AMAVs at first. 
Subsequently, this strategy constructs and prunes search trees to involve several steps of lookahead about BMAVs to plan each AMAV in a non-myopic manner according to the information-theoretic-based estimation uncertainty measurement about BMAVs.

We fully design and implement H-Swarm on heterogeneous MAV swarm consisting of industrial drones. 
% Then we conduct extensive experiments to evaluate H-Swarm's navigation success rate, localization accuracy, and latency. 
% Meanwhile, we evaluate the robustness of the H-Swarm under various conditions. 
Then we conduct extensive experiments to evaluate H-Swarm's performance and robustness. 
% We further evaluate the robustness of the H-Swarm under conditions of various numbers of AMAVs and BMAVs, the noise level of BMAVs' motion, and the noise level of AMAVs' observations. 
% The entire experiment lasts around 15 hours. 
We compare H-Swarm with three related works, including a reinforcement learning-based state-of-the-art (SOTA) solution.
The experiment results show that H-Swarm maintains an average localization error under $1m$, outperforming the other baselines by $>60\%$. H-Swarm also achieves a navigation success rate $>95\%$ on average, which has a 30\% improvement compared with the other baselines.
 % under given time and accuracy constraints
Moreover, H-Swarm runs in real-time compared with collaborative SLAM methods.

In summary, the main contributions are as follows:
\begin{itemize}
\item We propose H-Swarm, a new framework that transforms AMAVs into mobile localization infrastructures, enhancing localization accuracy and real-time performance for lightweight BMAVs, and thus promoting widespread swarm deployment.
    % \item We upgrade the localization paradigm of collaborative localization of heterogeneous MAV swarm so that the sensing resources of AMAVs can be fully utilized and used as the external mobile localization infrastructure of BMAVs, forming a large-scale, low-cost, high-precision, and real-time localization scheme suitable for heterogeneous MAV swarm.
\item We design an \textit{error-tolerant joint pose estimation} model and a \textit{graph-based adaptive grouping-scheduling} strategy to boost the pose optimization accuracy with noisy intermediate estimations and solve the resource allocation issues with dynamic coverage scenarios, respectively, making H-Swarm a practical solution for large-scale and low-cost MAV swarms. 
    % \item We propose the \textit{ETJE} model to estimate the location of BMAVs, which improves the localization accuracy and real-time performance of BMAVs, and the dependence of BMAVs on high-precision sensors and intensive computing resources is reduced, thus reducing the overall cost of the swarm and expanding the deployment range.
    % \item We design a novel graph-based adaptive grouping-scheduling strategy, which adaptively allocates sensing resources of AMAVs to achieve dynamic coverage of BMAVs. This strategy achieves a limited localization error and competitive navigation success rate.
\item We evaluate our solution through in-field experiments and large-scale physical feature-based simulations. Results show that our solution can localize BMAVs in real-time, achieving a 60\% reduction in localization error, and a 30\% improvement in navigation success rate.
\end{itemize}

The remainder of the paper is organized as follows: Section II presents the overview of H-Swarm, followed by detailed descriptions of the error-tolerant joint pose estimation model in Section III and graph-based adaptive grouping-scheduling strategy in Section IV.
The implementation and evaluation of our system are shown in Section V. 
We discuss the related work in Section VI and conclude H-Swarm in Section VII. We also attach several Appendix sections including detailed formula derivations of essential variables.


% \IEEEPARstart{E}{mergency} response operations are characterized by their complexity, which poses significant challenges for rescuers \cite{pal2020smartphone, shah2021multidimensional}. 
% Inefficient rescue operations may result from a lack of clear understanding about the extent of damage \cite{hong2021measuring}.
% To address this issue, a promising solution involves the use of Micro Aerial Vehicles (MAVs) to explore dangerous environments, such as those resulting from earthquakes \cite{golabi2017edge}, landslides \cite{ren2022color} and forest fires \cite{fouda2022lightweight}.
% By providing valuable environmental information, MAVs can enhance the effectiveness of rescue operations.

% The key components for effectively employing a MAVs swarm are localization and navigation, as highlighted in recent studies \cite{famili2022pilot, wang2022micnest, ruiz2016demo}. 
% To maintain localization accuracy during navigation, researchers propose various approaches. Some of these approaches rely on external infrastructures, such as GPS, radio, and motion capture devices \cite{chen2020distributed, chi2022wi, preiss2017crazyswarm}.
% In contrast, recent techniques employ advanced sensors, such as depth cameras or LiDARs, in conjunction with simultaneous localization and mapping (SLAM) methods \cite{zhang2022octoants, zhou2022swarm, loquercio2021learning}.

% \begin{figure}[t]
% \setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
% \setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
% \setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
% \centering
%     \subfigure[Earthquake]{
%         \centering
%             \includegraphics[width=0.3\columnwidth]{Figs/scenario1.pdf}
%         % \label{success100s}
%     }
%     \subfigure[Landslide]{
%         \centering
%             \includegraphics[width=0.3\columnwidth]{Figs/scenario2.pdf}
%         % \label{success0.2m}
%     }
%     \subfigure[Forest fire]{
%         \centering
%             \includegraphics[width=0.3\columnwidth]{Figs/scenario3.pdf}
%         % \label{success0.2m}
%     }
%     % \subfigure[Avalanche]{
%     %     \centering
%     %         \includegraphics[width=0.35\columnwidth]{Figs/scenario4.pdf}
%         % \label{success0.2m}
%     % }
% \caption{Example applications of MAV swarm.}
% \label{scenario}
% \vspace{-1.5em}
% \end{figure}

% Regrettably, the solutions mentioned above cannot be directly implemented in the context of emergency response for MAV swarms, owing to the following characteristics. 
% Firstly, the widespread deployment of a large-scale MAV swarm can significantly enhance efficiency by enabling simultaneous exploration, as reported in \cite{chen2020h}. 
% However, the highly dangerous nature of emergency scenarios renders the MAVs highly vulnerable to damage. 
% Consequently, to ensure survivability and reduce costs, the swarm is typically composed of low-cost, low-complexity nodes, as highlighted in \cite{chen2015drunkwalk}. 
% This, in turn, renders the utilization of SLAM methods infeasible for the swarm. 
% Secondly, an external localization infrastructure can be employed to provide reference signals to limit the localization error, as suggested in previous studies \cite{chi2022wi, wang2022h}. 
% However, in emergency response scenarios, the pre-existing infrastructure may be destroyed, rendering reference signals unavailable. 
% Moreover, the deployment of infrastructure in advance may be impractical or impossible in such situations.

% This paper tries to address the question: \textbf{How can a low-cost MAV swarm achieve precise localization and navigation without the aid of localization infrastructure?}
% The characteristics outlined above prompt us to explore the viability of integrating various localization techniques to develop a two-tier heterogeneous MAV swarm. This swarm is composed of two distinct types of MAVs:
% \textbf{(1) Basic MAVs (BMAVs)} - a significant number of resource-constrained MAVs, responsible for navigating toward destinations for the purpose of sensing. Their localization error tends to increase over time due to noisy measurements using conventional methods \cite{borenstein1996navigating}.
% \textbf{(2) Advanced MAVs (AMAVs)} - a small number of resource-intensive MAVs possess premium sensing capability to localize independently. The AMAV equips with forward-facing visual sensors to share sensing resources (generate observations) for BMAVs to limit localization error.
% The AMAVs serve as mobile localization infrastructure and share sensing resources to help localize BMAVs.
% The typical cost of AMAV and BMAV is 890\$ and 170\$, respectively.
% The AMAVs function as mobile infrastructure for localization and facilitate the localization of BMAVs by sharing sensing resources.
% With the assistance of a small number of AMAVs, the localization error of the whole swarm can be significantly reduced.
% Additionally, this swarm is relatively inexpensive to maintain, which enables its widespread deployment for rapid response.

% Since we share sensing resources of a small number AMAVs with a substantial quantity of BMAVs to limit localization errors, it is a non-trivial task to design an efficient sensing resource allocation strategy for AMAVs and faces two significant challenges.
% \textbf{(C1):}
% The objective of AMAVs is to share sensing resources with BMAVs which aims to enhance the localization of BMAVs. Nevertheless, in emergency response, the ground truth locations of BMAVs are unknown, thereby rendering the determination of the localization errors of BMAVs challenging. 
% This, in turn, complicates the sensing resources allocation of AMAVs.
% \textbf{(C2):}
% Simultaneously, different BMAVs exhibit varying locations and localization errors, while the distinct AMAVs possess varying locations, making sensing resources allocation of AMAVs an inherently intricate optimization problem.
% Furthermore, the quality of observations is influenced by the distance between the AMAV and the BMAV, which necessitates a trade-off between quantity and quality. 
% Additionally, the restricted velocity of AMAVs results in the displacement of BMAVs during the AMAV's travel to provide observations, which requires the AMAVs to account for this displacement, leading to a high computational cost \cite{kunze2018artificial}.
% As a result, the sensing resource allocation of AMAVs is a high-dimensional combinatorial optimization problem with a large search space.

% \begin{table}[]
% \centering
% \caption{The cost of the AMAV and the BMAV.}
% \begin{threeparttable}
% \begin{tabular}{cccccc}
% \hline
% \multicolumn{6}{c}{Cost of AMAV and BMAV (\$)}                                                                                        \\ \hline
% \multicolumn{1}{c|}{Type} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Auto-\\ pilot\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Embedded\\ computer\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Optical\\ Flow\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Tracking \\ camera\end{tabular}} & All  \\ \hline

% \multicolumn{1}{c|}{AMAV\tnote{*}} & \multicolumn{1}{c|}{400}                                                   & \multicolumn{1}{c|}{800}                                                          & \multicolumn{1}{c|}{/}                                       & \multicolumn{1}{c|}{324}                                                        & 1524 \\ \hline
% \multicolumn{1}{c|}{BMAV\tnote{**}} & \multicolumn{1}{c|}{200}                                                   & \multicolumn{1}{c|}{/}                                             & \multicolumn{1}{c|}{50}                                                     & \multicolumn{1}{c|}{/}                                           & 250  \\ \hline
% \end{tabular}

% \begin{tablenotes}
%     \footnotesize
%     \item[*] The AMAV consists of Pixhawk 4 autopilot, Nvidia Jetson Xavier NX embedded computer, Intel realsense T265 tracking camera. All data are from https://www.amazon.com.
%     \item[**] The BMAV is based on Bitcraze Crazyflie nano quadcopter, and the data are from https://store.bitcraze.io/.
% \end{tablenotes}
% \end{threeparttable}
% \label{cost}
% \vspace{-2.0em}
% \end{table}

% This paper presents a novel active planning-based resource allocation system, denoted as \textit{H-Swarm}, which overcomes the above issues. 
% \textbf{To address the challenge (C1)}, the measure of information, obtained from the covariance matrix trace of BMAVs' location estimation, serves as a reflection of the quality of BMAVs' location estimations, rather than the localization error. 
% \textit{H-Swarm} employs this indicator to allocate the sensing resources of AMAVs to BMAVs through planning. 
% \textbf{To address the challenge (C2)}, \textit{H-Swarm} sacrifice some observation model accuracy via linearization to reduce the computational complexity in location estimation of BMAVs at first.
% Subsequently, the distance between AMAVs and the location estimation of BMAVs is utilized to dynamically group the AMAVs and BMAVs.
% Following the grouping, each AMAV shares sensing resources for nearby BMAVs to avoid flights that do not generate observations, thereby conserving the AMAV's sensing resources.
% Subsequently, \textit{H-Swarm} constructs search trees for non-myopic planning of each AMAV to generate observations for corresponding BMAVs.   
% This planning involves several steps of lookahead about the BMAVs assigned to each AMAV. 
% To further reduce search time, \textit{H-Swarm} discards some but not all of the nodes at each level of the search tree of each AMAV based on the similarity of nodes in AMAV's location and estimation covariance about BMAVs assigned to it.

% We summarize our contributions as follows.
% \begin{itemize}
%     \item We propose a heterogeneous MAV swarm-based extreme environment sensing system which can be widely deployed without localization infrastructure.
%     % \item We utilize a measure of information to reflect the quality of location estimations of BMAVs instead of localization error, which efficiently guides the planning of AMAVs to allocate observational resources to help BMAVs' localization.
%     \item We utilize a measure of information to reflect the quality of location estimations, which effectively guides the AMAVs to limit the localization error of BMAVs.
%     \item We propose a resource allocation system (\textit{H-Swarm}) to adaptively group the AMAVs and BMAVs and plan the AMAVs with the non-myopic objective collaboratively.
%     \item We evaluate our solution through in-field experiment and large-scale physical feature-based simulations. Results show that our solution achieves a 64\% reduction on average in localization error, and as much as 30\% improvement in navigation success rate under given time and accuracy constrain.
% \end{itemize}

% The remainder of the paper is organized as follows: Section \ref{3} presents the sensing system based on heterogeneous MAV swarm and problem definition. Section \ref{4} introduces \textit{H-Swarm}, including an overview and corresponding algorithms. Section \ref{5} demonstrates experimental results. Section \ref{2} summarizes related work. Section \ref{6} concludes the paper.


 


















==> intro_backup.tex <==
\section{Introduction}
% MAV for emergency response is a new trend....
% \IEEEPARstart{E}{mergency} response is considered extreme for rescuers due to the complexity of the environment \cite{pal2020smartphone, shah2021multidimensional}. 
\IEEEPARstart{E}{mergency} response operations are characterized by their complexity, which poses significant challenges for rescuers \cite{pal2020smartphone, shah2021multidimensional}. 
Inefficient rescue operations may result from a lack of clear understanding about the extent of damage \cite{hong2021measuring}.
To address this issue, a promising solution involves the use of Micro Aerial Vehicles (MAVs) to explore dangerous environments, such as those resulting from earthquakes \cite{golabi2017edge}, landslides \cite{ren2022color} and forest fires \cite{fouda2022lightweight}.
By providing valuable environmental information, MAVs can enhance the effectiveness of rescue operations.

The key components for effectively employing a MAVs swarm are localization and navigation, as highlighted in recent studies \cite{famili2022pilot, wang2022micnest, ruiz2016demo}. 
To maintain localization accuracy during navigation, researchers propose various approaches. Some of these approaches rely on external infrastructures, such as GPS, radio, and motion capture devices \cite{chen2020distributed, chi2022wi, preiss2017crazyswarm}.
In contrast, recent techniques employ advanced sensors, such as depth cameras or LiDARs, in conjunction with simultaneous localization and mapping (SLAM) methods \cite{zhang2022octoants, zhou2022swarm, loquercio2021learning}.

% \begin{figure}[t]
% \setlength{\abovecaptionskip}{0.cm} % height above Figure X caption
% \setlength{\belowcaptionskip}{-0.4cm} % height between Figure X caption and text main body. set to -0.4 at most, more leads to overlap
% \setlength{\subfigcapskip}{-0.1cm}  % height between subfigure (x) and its subscription
% \centering
%     \subfigure[Earthquake]{
%         \centering
%             \includegraphics[width=0.3\columnwidth]{Figs/scenario1.pdf}
%         % \label{success100s}
%     }
%     \subfigure[Landslide]{
%         \centering
%             \includegraphics[width=0.3\columnwidth]{Figs/scenario2.pdf}
%         % \label{success0.2m}
%     }
%     \subfigure[Forest fire]{
%         \centering
%             \includegraphics[width=0.3\columnwidth]{Figs/scenario3.pdf}
%         % \label{success0.2m}
%     }
%     % \subfigure[Avalanche]{
%     %     \centering
%     %         \includegraphics[width=0.35\columnwidth]{Figs/scenario4.pdf}
%         % \label{success0.2m}
%     % }
% \caption{Example applications of MAV swarm.}
% \label{scenario}
% \vspace{-1.5em}
% \end{figure}

Regrettably, the solutions mentioned above cannot be directly implemented in the context of emergency response for MAV swarms, owing to the following characteristics. 
Firstly, the widespread deployment of a large-scale MAV swarm can significantly enhance efficiency by enabling simultaneous exploration, as reported in \cite{chen2020h}. 
However, the highly dangerous nature of emergency scenarios renders the MAVs highly vulnerable to damage. 
Consequently, to ensure survivability and reduce costs, the swarm is typically composed of low-cost, low-complexity nodes, as highlighted in \cite{chen2015drunkwalk}. 
This, in turn, renders the utilization of SLAM methods infeasible for the swarm. 
Secondly, an external localization infrastructure can be employed to provide reference signals to limit the localization error, as suggested in previous studies \cite{chi2022wi, wang2022h}. 
However, in emergency response scenarios, the pre-existing infrastructure may be destroyed, rendering reference signals unavailable. 
Moreover, the deployment of infrastructure in advance may be impractical or impossible in such situations.

This paper tries to address the question: \textbf{How can a low-cost MAV swarm achieve precise localization and navigation without the aid of localization infrastructure?}
The characteristics outlined above prompt us to explore the viability of integrating various localization techniques to develop a two-tier heterogeneous MAV swarm. This swarm is composed of two distinct types of MAVs:
\textbf{(1) Basic MAVs (BMAVs)} - a significant number of resource-constrained MAVs, responsible for navigating toward destinations for the purpose of sensing. Their localization error tends to increase over time due to noisy measurements using conventional methods \cite{borenstein1996navigating}.
\textbf{(2) Advanced MAVs (AMAVs)} - a small number of resource-intensive MAVs possess premium sensing capability to localize independently. The AMAV equips with forward-facing visual sensors to share sensing resources (generate observations) for BMAVs to limit localization error.
% The AMAVs serve as mobile localization infrastructure and share sensing resources to help localize BMAVs.
The typical cost of AMAV and BMAV is 890\$ and 170\$, respectively.
The AMAVs function as mobile infrastructure for localization and facilitate the localization of BMAVs by sharing sensing resources.
With the assistance of a small number of AMAVs, the localization error of the whole swarm can be significantly reduced.
Additionally, this swarm is relatively inexpensive to maintain, which enables its widespread deployment for rapid response.

Since we share sensing resources of a small number AMAVs with a substantial quantity of BMAVs to limit localization errors, it is a non-trivial task to design an efficient sensing resource allocation strategy for AMAVs and faces two significant challenges.
\textbf{(C1):}
The objective of AMAVs is to share sensing resources with BMAVs which aims to enhance the localization of BMAVs. Nevertheless, in emergency response, the ground truth locations of BMAVs are unknown, thereby rendering the determination of the localization errors of BMAVs challenging. 
This, in turn, complicates the sensing resources allocation of AMAVs.
\textbf{(C2):}
Simultaneously, different BMAVs exhibit varying locations and localization errors, while the distinct AMAVs possess varying locations, making sensing resources allocation of AMAVs an inherently intricate optimization problem.
% Moreover, the AMAV has a limited field of view, and the noise of observation is contingent on the distance between the AMAV and the BMAV, which facilitates a trade-off between quantity and quality.
Furthermore, the quality of observations is influenced by the distance between the AMAV and the BMAV, which necessitates a trade-off between quantity and quality. 
Additionally, the restricted velocity of AMAVs results in the displacement of BMAVs during the AMAV's travel to provide observations, which requires the AMAVs to account for this displacement, leading to a high computational cost \cite{kunze2018artificial}.
As a result, the sensing resource allocation of AMAVs is a high-dimensional combinatorial optimization problem with a large search space.

% \begin{table}[]
% \centering
% \caption{The cost of the AMAV and the BMAV.}
% \begin{threeparttable}
% \begin{tabular}{cccccc}
% \hline
% \multicolumn{6}{c}{Cost of AMAV and BMAV (\$)}                                                                                        \\ \hline
% \multicolumn{1}{c|}{Type} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Auto-\\ pilot\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Embedded\\ computer\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Optical\\ Flow\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Tracking \\ camera\end{tabular}} & All  \\ \hline

% \multicolumn{1}{c|}{AMAV\tnote{*}} & \multicolumn{1}{c|}{400}                                                   & \multicolumn{1}{c|}{800}                                                          & \multicolumn{1}{c|}{/}                                       & \multicolumn{1}{c|}{324}                                                        & 1524 \\ \hline
% \multicolumn{1}{c|}{BMAV\tnote{**}} & \multicolumn{1}{c|}{200}                                                   & \multicolumn{1}{c|}{/}                                             & \multicolumn{1}{c|}{50}                                                     & \multicolumn{1}{c|}{/}                                           & 250  \\ \hline
% \end{tabular}

% \begin{tablenotes}
%     \footnotesize
%     \item[*] The AMAV consists of Pixhawk 4 autopilot, Nvidia Jetson Xavier NX embedded computer, Intel realsense T265 tracking camera. All data are from https://www.amazon.com.
%     \item[**] The BMAV is based on Bitcraze Crazyflie nano quadcopter, and the data are from https://store.bitcraze.io/.
% \end{tablenotes}
% \end{threeparttable}
% \label{cost}
% \vspace{-2.0em}
% \end{table}

This paper presents a novel active planning-based resource allocation system, denoted as \textit{H-Swarm}, which overcomes the above issues. 
\textbf{To address the challenge (C1)}, the measure of information, obtained from the covariance matrix trace of BMAVs' location estimation, serves as a reflection of the quality of BMAVs' location estimations, rather than the localization error. 
\textit{H-Swarm} employs this indicator to allocate the sensing resources of AMAVs to BMAVs through planning. 
\textbf{To address the challenge (C2)}, \textit{H-Swarm} sacrifice some observation model accuracy via linearization to reduce the computational complexity in location estimation of BMAVs at first.
Subsequently, the distance between AMAVs and the location estimation of BMAVs is utilized to dynamically group the AMAVs and BMAVs.
Following the grouping, each AMAV shares sensing resources for nearby BMAVs to avoid flights that do not generate observations, thereby conserving the AMAV's sensing resources.
Subsequently, \textit{H-Swarm} constructs search trees for non-myopic planning of each AMAV to generate observations for corresponding BMAVs.   
This planning involves several steps of lookahead about the BMAVs assigned to each AMAV. 
To further reduce search time, \textit{H-Swarm} discards some but not all of the nodes at each level of the search tree of each AMAV based on the similarity of nodes in AMAV's location and estimation covariance about BMAVs assigned to it.

We summarize our contributions as follows.
\begin{itemize}
    \item We propose a heterogeneous MAV swarm-based extreme environment sensing system which can be widely deployed without localization infrastructure.
    % \item We utilize a measure of information to reflect the quality of location estimations of BMAVs instead of localization error, which efficiently guides the planning of AMAVs to allocate observational resources to help BMAVs' localization.
    \item We utilize a measure of information to reflect the quality of location estimations, which effectively guides the AMAVs to limit the localization error of BMAVs.
    \item We propose a resource allocation system (\textit{H-Swarm}) to adaptively group the AMAVs and BMAVs and plan the AMAVs with the non-myopic objective collaboratively.
    \item We evaluate our solution through in-field experiment and large-scale physical feature-based simulations. Results show that our solution achieves a 64\% reduction on average in localization error, and as much as 30\% improvement in navigation success rate under given time and accuracy constrain.
\end{itemize}

The remainder of the paper is organized as follows: Section \ref{3} presents the sensing system based on heterogeneous MAV swarm and problem definition. Section \ref{4} introduces \textit{H-Swarm}, including an overview and corresponding algorithms. Section \ref{5} demonstrates experimental results. Section \ref{2} summarizes related work. Section \ref{6} concludes the paper.


 


















==> systemmodel_bk.tex <==
\section{System Model and Problem Definition}\label{3}
% In this section, we will present the heterogeneous MAV swarm-based environmental sensing system-\textit{H-Swarm}.
% Specifically, we first introduce the architecture 
% In this section, we will introduce how the sensing resource allocation problem is formulated to optimize the path planning of AMAVs for the localization of BMAVs.
% Specifically, we first present the architecture of the sensing system in Section \ref{3.1}.
% Then, we introduce the preliminary definition and background in Section \ref{3.2}.
% Subsequently, we discuss the objective of limiting the localization error of BMAVs in Section \ref{3.3}.
% Finally, we formulate the problem of sensing resource allocation in Section \ref{3.4}.

In this section, we introduce the formulation of the sensing resource allocation problem to optimize the path planning of AMAVs for localizing BMAVs.
We present the sensing system's architecture in Section \ref{3.1}, followed by introducing preliminary definitions and background in Section \ref{3.2}.
Next, we discuss the objective of limiting the localization error of BMAVs in Section \ref{3.3} before formulating the problem of sensing resource allocation in Section \ref{3.4}.

\subsection{Operation and Architecture}\label{3.1}
\begin{figure}[t]
    \centering
        \includegraphics[width=1\columnwidth]{Figs/sensingsys.pdf}
    \caption{Architecture of the heterogeneous MAV swarm-based extreme environment sensing system, which is composed of three subsystems.}
    \label{sensingsys}
    \vspace{-0.4cm}
\end{figure} 

% Fig. \ref{sensingsys} illustrates the architecture of the heterogeneous MAV swarm-based sensing system, which consists of four subsystems including the \textit{Heterogeneous MAV swarm}, the \textit{Resource Allocation System}, the \textit{Data Request End}, and the \textit{Application System}. 

% Fig. \ref{sensingsys} illustrates the architecture of the heterogeneous MAV swarm-based sensing system, which consists of three subsystems including the \textit{Heterogeneous MAV swarm}, the \textit{Resource Allocation System}, and the \textit{Data Request End}. 
% In this section, we introduce each part of the system as follows.
% The \textit{Data Request End} submits data requirements to the \textit{resource allocation System} \cite{yu2020disruption}. 
% The \textit{Heterogeneous MAV swarm} sends collected data to the \textit{Data Request End} for further analysis. 
% Based on the analysis results, the \textit{Data Request End} maps the phenomena of common interest, which is used for decision-making of further data requirements \cite{xu2022seismic}.

% The \textit{Heterogeneous MAV swarm} consists of a large number of BMAVs and a small amount of AMAVs. 
% The BAMVs are equipped with various sensors according to the sensing requirement, such as pollution detectors \cite{sun2022c}. However, with limited sensing capability and traditional methods, the localization error of BMAVs increases over time. 
% The AMAVs can localize themselves with advanced sensing capabilities and help limit localization errors of BMAVs.

% The \textit{Resource Allocation System} schedules a large number of BMAVs to designated destinations to collect the sensing data, while navigating a small amount of AMAVs to assist the BAMVs in localization.
% In this work, the \textit{Resource Allocation System} mainly focuses on sensing resource allocation through the planning of AMAVs, while the destinations of BMAVs are considered to be given in advance.
% In this way, the BMAVs can be considered mobile sensors, while AMAVs can be considered mobile localization infrastructure for BAMVs. 
% This system takes location information from the \textit{Heterogeneous MAV swarm}, including motion measurement of BMAVs and observation from AMAVs.
% Then, it decides (1) For a BMAV, which AMAV should be chosen to help it, (2) For an AMAV, how it be planned to allocate sensing resources to help multiple BAMVs and send motion commands to them.
% The \textit{Resource Allocation System} is not dependent on particular applications, and it can be used for various sensing tasks by replacing sensors in BMAVs.


Fig. \ref{sensingsys} shows the heterogeneous MAV swarm-based sensing system's architecture, including three subsystems: the \textit{Heterogeneous MAV swarm}, the \textit{Resource Allocation System}, and the \textit{Data Request End}.
% We introduce each part of the system in this part.

The \textit{Data Request End} submits data requirements to the \textit{Resource Allocation System} \cite{yu2020disruption}, while the \textit{Heterogeneous MAV swarm} sends collected data to the \textit{Data Request End} for further analysis.
With the analysis results, the \textit{Data Request End} maps phenomena of common interest, used for decision-making of further data requirements \cite{xu2022seismic}.

The \textit{Heterogeneous MAV swarm} includes a large number of BMAVs, equipped with varied sensors based on sensing requirements, and a small amount of AMAVs.
However, with limited sensing capability and traditional methods, the localization error of BMAVs increases over time, while AMAVs can localize themselves with advanced sensing capabilities and limit localization errors of BMAVs.

The \textit{Resource Allocation System} schedules a large number of BMAVs to designated destinations for sensing data collection, and navigates a small amount of AMAVs to assist BMAVs in localization \cite{sun2022c}.
This system focuses on sensing resource allocation through the planning of AMAVs while considering given destinations of BMAVs.
BMAVs can be considered mobile sensors, while AMAVs can be mobile localization infrastructure for BMAVs.
The system takes location information from the \textit{Heterogeneous MAV swarm}, (1) decides which AMAVs should assist which BMAVs, and (2) plans and allocates sensing resources for multiple BMAVs by sending motion commands to AMAVs.
It operates independently of various sensing tasks and can be used by replacing sensors on BMAVs.

\subsection{Background and Key definitions}\label{3.2}
% In this section, we define several key concepts and summarize main notations and descriptions in Appendix \ref{notation}.

\subsubsection{Environmental Description} 
% Consider a bounded space $\Omega \in \mathbb{R}^3$ whose length, width, and height are $L$, $W$, and $H$. 
% The heterogeneous MAV swarm operates in $\Omega$.
% This heterogeneous MAV swarm contains multiple BMAVs and AMAVs, which operate independently, the number of BMAVs and AMAVs does not change during the operation. 
% For simplicity of analysis, BMAVs and AMAVs are both operating at the same altitude in this paper. 
% By increasing the velocity perpendicular to the ground, the heterogeneous MAV swarm can be introduced to three-dimensional space.
Let $\Omega$ be a bounded space in $\mathbb{R}^3$ with length, width, and height $L$, $W$, and $H$, respectively, where the heterogeneous MAV swarm operates.
This swarm comprises a fixed number of BMAVs and AMAVs that operate independently. 
For simplicity, we assume that both types of MAVs operate at the same altitude in this paper.
By increasing the velocity perpendicular to the ground, the swarm can operate in three-dimensional space.

\subsubsection{State model of AMAV} 
% There are $M$ ($M$ \textgreater $1$) AMAVs in a heterogeneous MAV swarm, where the $j$-th AMAV is represented by $A_j$.
% The state of $A_j$ at time $t$ is formed by location and motion command at time $t$. 
% The location is $\boldsymbol{x_{j, t}}=(x_{j,t}^1, x_{j,t}^2, \phi_{j,t})$, where $\phi_{j,t})$ is orient angle.
% The metric $d_{\chi}$ measures the distance between two locations.
% The motion command is $\boldsymbol{u_{j, t}} = (u_{j,t}, \omega_{j,t})$, where $u_{j,t}$ is the translational velocity and $\omega_{j,t}$ is the rotational velocity.
% The AMAV obeys the following motion model, 
% \begin{equation}
% \boldsymbol{x_{j, t}} = f(\boldsymbol{x_{j, t-1}}, \boldsymbol{u_{j, t-1}}). \\
% \end{equation}
% The AMAV can obtain accurate location estimation with its advanced sensing capabilities. Specifically, the motion model of AMAV can be expressed in the following form,
% \begin{equation}
% \left(\begin{array}{c}
% x_{j,t}^1\\
% x_{j,t}^2\\
% \phi_{j,t}
% \end{array}\right)=\left(\begin{array}{l}
% x_{j,t-1}^1\\
% x_{j,t-1}^2\\
% \phi_{j,t-1}
% \end{array}\right) + \left(\begin{array}{c}
% u_{j,t-1} \cos \left(\phi_{j,t-1}\right) \\
% u_{j,t-1} \sin \left(\phi_{j,t-1}\right) \\
% \omega_{j,t-1}
% \end{array}\right).
% \end{equation}
The heterogeneous MAV swarm contains $M$ ($M\textgreater1$) AMAVs denoted as $A_j$, with each AMAV's state at time $t$ consisting of location and motion command.
The location is represented by $\boldsymbol{x_{j,t}}=(x_{j,t}^1, x_{j,t}^2, \phi_{j,t})$, where $\phi_{j,t}$ is the orient angle, and the distance between two locations is measured using the metric $d_{\chi}$. For motion command, $\boldsymbol{u_{j, t}} = (u_{j,t}, \omega_{j,t})$, where $u_{j,t}$ and $\omega_{j,t}$ are the translational and rotational velocities, respectively.
The AMAVs follow the motion model expressed as $\boldsymbol{x_{j, t}} = f(\boldsymbol{x_{j, t-1}}, \boldsymbol{u_{j, t-1}})$ and can accurately estimate their location using advanced sensing capabilities.
Specifically, the motion model for an AMAV can be represented as follows:
\begin{equation}
\left(\begin{array}{c}
x_{j,t}^1 \\
x_{j,t}^2 \\
\phi_{j,t}
\end{array}\right) =
\left(\begin{array}{c}
x_{j,t-1}^1 \\
x_{j,t-1}^2 \\
\phi_{j,t-1}
\end{array}\right) + \left(\begin{array}{c}
u_{j,t-1} \cos \left(\phi_{j,t-1}\right) \\
u_{j,t-1} \sin \left(\phi_{j,t-1}\right) \\
\omega_{j,t-1}
\end{array}\right).
\end{equation}

\subsubsection{State model of BMAV} 
% There are $N$ ($N$ \textgreater $1$) BMAVs in a heterogeneous MAV swarm, where the $i$-th BMAV is represented by $B_i$.
% The state of $B_i$ at time $t$ is formed by location and motion command at time $t$. The location is $\boldsymbol{y_{i, t}}=(y_{i,t}^1, y_{i,t}^2)$ and the motion command is $\boldsymbol{v_{i, t}} = (v_{i,t}^1, v_{i,t}^2)$.
% The $B_i$ follows double integrator dynamics with Gaussian noise as follows, 
% \begin{equation}
% \begin{gathered}
% \left(\begin{array}{l}
% y_{i, t+\delta}^1 \\
% y_{i, t+\delta}^2
% \end{array}\right)=\left(\begin{array}{l}
% y_{i, t}^1 \\
% y_{i, t}^2
% \end{array}\right)+\delta\left(\begin{array}{l}
% v_{i, t}^1+n_{i, t}^1 \\
% v_{i, t}^2+n_{i, t}^2
% \end{array}\right),\\
% \text{$n_{i, t}^1$ is drawn from $p(n^1)$,} \\
% \text{$n_{i, t}^2$ is drawn from $p(n^2)$,}
% \end{gathered}
% \label{y}
% \end{equation}
% where the $p(n^1)$ and $p(n^2)$ are motion noise models and $\delta$ ($\delta > 1$) is time interval between two commands.
% The $p(n^1)$ and $p(n^2)$ are empirically obtained from our test MAV platform but can be specified according to the MAV platform used. 
% According to \cite{chen2020h}, $p(n^1)$ and $p(n^2)$ are specified as normal distributions with mean $\mu = 0$ and variance $\sigma$ is expressed as a percentage of $v_{i, t}^1$ and $v_{i, t}^2$.
% Due to the limited onboard capability and the lack of localization infrastructure, the \textit{Resource Allocation System} cannot obtain actual locations and motion commands of BMAVs.
% Instead, it maintains the location estimation of $B_i$ $\boldsymbol{\widehat{y}_{i, t}}$ using the noisy motion measurements $\boldsymbol{\dot{v}_{i, t}}$ from inertial measurement unit (IMU) of $B_i$.
% The covariance matrix of location estimation at time $t$ is $\Sigma_{i, t}$.


The heterogeneous MAV swarm includes $N$ ($N\textgreater1$) BMAVs referred to as $B_i$, with the state of $B_i$ at time $t$ consisting of location and motion command.
The location of $B_i$ is $\boldsymbol{y_{i, t}}=(y_{i,t}^1, y_{i,t}^2)$, and its motion command is $\boldsymbol{v_{i, t}} = (v_{i,t}^1, v_{i,t}^2)$.
$B_i$ follows double integrator dynamics with Gaussian noise represented as follows:
\begin{equation}
\begin{gathered}
\left(\begin{array}{l}
y_{i, t+\delta}^1 \\
y_{i, t+\delta}^2
\end{array}\right)=\left(\begin{array}{l}
y_{i, t}^1 \\
y_{i, t}^2
\end{array}\right)+\delta\left(\begin{array}{l}
v_{i, t}^1+n_{i, t}^1 \\
v_{i, t}^2+n_{i, t}^2
\end{array}\right),\\
\text{$n_{i, t}^1$ is drawn from $p(n^1)$,} \\
\text{$n_{i, t}^2$ is drawn from $p(n^2)$,}
\end{gathered}
\label{y}
\end{equation}
where $n_{i, t}^1$ and $n_{i, t}^2$ are drawn from motion noise models $p(n^1)$ and $p(n^2)$ respectively, $\delta$ ($\delta > 1$) denotes the time interval between two commands.
The motion noise models $p(n^1)$ and $p(n^2)$ empirically obtaining from testbed are specified as normal distributions with mean $\mu = 0$ and variance $\sigma$, expressed as a percentage of $v_{i, t}^1$ and $v_{i, t}^2$, as outlined in \cite{chen2020h}.
Due to limited onboard capability and the absence of localization infrastructure, the \textit{Resource Allocation System} cannot obtain actual locations and motion commands of the BMAVs.
Instead, it estimates the location of $B_i$ as $\boldsymbol{\widehat{y}_{i, t}}$ using the noisy motion measurements $\boldsymbol{\dot{v}_{i, t}}$ from an inertial measurement unit (IMU) on $B_i$.
The location estimation at time $t$ is represented by the covariance matrix $\Sigma_{i, t}$.


\subsubsection{Observation model of AMAV:}
As Fig. \ref{observation} illustrates, $A_j$ is equipped with a visual sensor that can generate observations for BMAVs with respect to their actual locations.
The observation angle of the visual sensor is denoted by $\phi$, and the field of view (FoV) of $A_j$ at time $t$ is defined as follows,
\begin{equation}
\begin{aligned}
& F_{j, t}=\{(x, y) \mid \\
& \quad \quad 0<\sqrt{\left(y-x_{j,t}^2\right)^2+\left(x-x_{j,t}^1\right)^2}<r_m \quad \bigcap \\
& \quad -\frac{\phi}{2}<\arctan\left(\left(y-x_{j,t}^2\right)\left(x-x_{j,t}^1\right)\right)-\phi<\frac{\phi}{2}\}, 
\end{aligned}
\label{F_t}
\end{equation}
where $r_m$ is the maximum distance that the sensor can observe, which is limited by the observation technique.

When $B_i$ in the FoV of $A_j$ at time $t$, $A_j$ generates noisy observation $z_{i, j, t}$ for $B_i$, which consists of range $r_{i, j, t}$ and bearing $\alpha_{i, j, t}$  for $B_i$, both $r_{i, j, t}$ and $\alpha_{i, j, t}$ are relative to $A_i$,
\begin{equation}
\begin{gathered}
\begin{aligned}
z_{i, j, t}
&=h(\boldsymbol{x_{j, t}}, \boldsymbol{y_{i, t}}) + \boldsymbol{n_{i, j, t}},\\
h(\boldsymbol{x_{j, t}}, \boldsymbol{y_{i, t}})
&:=\left[\begin{array}{c}
% r(\boldsymbol{x}, \boldsymbol{y})  \\
% \alpha(\boldsymbol{x}, \boldsymbol{y})
r_{i, j, t} \\
\alpha_{i, j, t}
\end{array}\right]\\
&:=\left[\begin{array}{c}
\sqrt{\left(y_{i, t}^1-x_{j, t}^1\right)^2+\left(y_{i, t}^2-x_{j, t}^2\right)^2} \\
\arctan \left(\left(y_{i, t}^2-x_{j, t}^2\right)\left(y_{i, t}^1-x_{j, t}^1\right)\right)-\phi
\end{array}\right]\\
\boldsymbol{n_{i, j, t}}
&:= [n_{i, j, t}^r, n_{i, j, t}^\alpha]^T
\end{aligned},\\
\text{$n_{i, j, t}^r$ is drawn from $p(n^r)$}, \\
\text{$n_{i, j, t}^\alpha$ is drawn from $p(n^\alpha)$}.
\end{gathered}
\label{z}
\end{equation}
% The $p(n^r)$ is the range measurement noise model and the $p(n^\alpha)$ is the bearing measurement noise model. 
% The $p(n^r)$ and $p(n^\alpha)$ are empirically obtained from out test heterogeneous MAV platform.
% In this work, $p(n^r)$ is specified as normal distributions with $\mu = 0$, and $\sigma$ is expressed as a percentage of $r_{i, j, t}$.
% The $p(n^\alpha)$ is specified as normal distributions with $\mu = 0$, and $\sigma$ is a constant cause the bearing measurement noise doesn't change depending on the bearing between $A_j$ and $B_i$ according to \cite{kalaitzakis2021fiducial}.
The noise models for range and bearing measurements are denoted as $p(n^r)$ and $p(n^\alpha)$, respectively, and are empirically obtained from our testbed.
For range measurements, $p(n^r)$ is specified as a normal distribution with mean $\mu = 0$ and variance $\sigma$, expressed as a percentage of $r_{i, j, t}$.
For bearing measurements, $p(n^\alpha)$ is also specified as a normal distribution with mean $\mu = 0$ and a constant variance, as the bearing measurement noise does not depend on the bearing between $A_j$ and $B_i$, as shown in \cite{kalaitzakis2021fiducial}.

% \textit{5) Prediction of BMAV from Motion Models: }
% The \textit{Scheduling System} utilizes noisy velocity measurement of BMAV $B_i$ $\boldsymbol{\dot{v}_{i, t}} = (\dot{v}_{i,t}^1, \dot{v}_{i,t}^2)$ to calculate the prior of $B_i$'s location at time $t$, which is specified as $\boldsymbol{{y_{i, t}}^{-}}=({y_{i,t}^1}^{-}, {y_{i,t}^2}^{-})$. The $\boldsymbol{{y_{i, t}}^{-}}$ is calculated as follow, 
% \begin{equation}
% \begin{gathered}
% \left(\begin{array}{l}
% {y_{i,t}^1}^{-} \\
% {y_{i,t}^2}^{-}
% \end{array}\right)=\left(\begin{array}{l}
% \widehat{y}_{i,t - 1}^1 \\
% \widehat{y}_{i,t - 1}^2
% \end{array}\right)+\left(\begin{array}{l}
% \dot{v}_{i,t}^1 \\
% \dot{v}_{i,t}^2
% \end{array}\right),\\
% \end{gathered}
% \end{equation}
% where $\boldsymbol{\widehat{y}_{i, t - 1}}=(\widehat{y}_{i,t - 1}^1, \widehat{y}_{i,t - 1}^2)$ is the estimation of $B_i$'s location at time $t - 1$.
% The covariance matrix of this prior is ${\Sigma_{i, t}}^-$.

% \textit{6) Correction of BMAV from Observations:} When BMAV $B_i$ in the FOV of the AMAV $A_j$ at time $t$, the \textit{Scheduling System} utilizes the observation $z_{i, j, t}$ generated by $A_j$ to calculate the posterior of the $B_i$'s location $\boldsymbol{{y_{i, t}}^{+}}=({y_{i,t}^1}^{+}, {y_{i,t}^2}^{+})$ with variant of Kalman filter. 
% The covariance matrix of this posterior is ${\Sigma_{i, t}}^+$.
% The detail of the calculation will be further introduced in \textcolor{red}{Section IV}. 
% Finally, the \textit{Scheduling System} calculates the estimation and covariance matrix of $B_i$'s location at time $t$, 
% \begin{equation}
%     \boldsymbol{\widehat{y}_{i,t}}=\{\begin{array}{l}\boldsymbol{{y_{i, t}}^{+}}, 
%     \text { if }  \mathrm{B}_{\mathrm{i}} \text{ in the FOV of } 
%     \mathrm{A}_{\mathrm{j}} \\ 
%     \boldsymbol{{y_{i, t}}^{-}}, 
%     \text { if } 
%     \mathrm{B}_{\mathrm{i}} \text{ not in the FOV of } \mathrm{A}_{\mathrm{j}}
%     \end{array}, 
% \end{equation}

% \begin{equation}
%     \Sigma_{i, t}=\{\begin{array}{l}{\Sigma_{i, t}}^-, 
%     \text { if }  \mathrm{B}_{\mathrm{i}} \text{ in the FOV of } 
%     \mathrm{A}_{\mathrm{j}} \\ 
%     {\Sigma_{i, t}}^+, 
%     \text { if } 
%     \mathrm{B}_{\mathrm{i}} \text{ not in the FOV of } \mathrm{A}_{\mathrm{j}}
%     \end{array}.
% \end{equation}

To simplify notation, we let
% \boldsymbol{B} := [B_1, \dots, B_N]\boldsymbol{B} := [B_1, \dots, B_N], 
% \boldsymbol{A} := [A_1, \dots, A_M]\boldsymbol{A} := [A_1, \dots, A_M], 
$\boldsymbol{y_t} := {[\boldsymbol{y_{1, t}^T}, \dots, \boldsymbol{y_{N, t}^T}]}^T$, 
% \boldsymbol{v_t} := {[\boldsymbol{v_{1, t}^T}, \dots, \boldsymbol{v_{N, t}^T}]}^T\boldsymbol{v_t} := {[\boldsymbol{v_{1, t}^T}, \dots, \boldsymbol{v_{N, t}^T}]}^T, 
% \boldsymbol{\dot{v}_t} := {[\boldsymbol{\dot{v}_{1, t}^T}, \dots, \boldsymbol{\dot{v}_{N, t}^T}]}^T\boldsymbol{\dot{v}_t} := {[\boldsymbol{\dot{v}_{1, t}^T}, \dots, \boldsymbol{\dot{v}_{N, t}^T}]}^T, 
$\boldsymbol{x_t} := {[\boldsymbol{x_{1, t}^T}, \dots, \boldsymbol{x_{M, t}^T}]}^T$, 
$\boldsymbol{u_t} := {[\boldsymbol{u_{1, t}^T}, \dots, \boldsymbol{u_{M, t}^T}]}^T$, 
% % \boldsymbol{z_{j, t}} := {[\boldsymbol{z_{1, j, t}^T}, \dots, \boldsymbol{z_{N, j, t}^T}]}^T\boldsymbol{z_{j, t}} := {[\boldsymbol{z_{1, j, t}^T}, \dots, \boldsymbol{z_{N, j, t}^T}]}^T, 
$\boldsymbol{\widehat{y}_t} := {[\boldsymbol{\widehat{y}_{1, t}^T}, \dots, \boldsymbol{\widehat{y}_{N, t}^T}]}^T$, 
% % \boldsymbol{y_t}^{-} := {[\boldsymbol{y_{1, t}^T}^{-}, \dots, \boldsymbol{y_{N, t}^T}^{-}]}^T\boldsymbol{y_t}^{-} := {[\boldsymbol{y_{1, t}^T}^{-}, \dots, \boldsymbol{y_{N, t}^T}^{-}]}^T, 
% % \boldsymbol{y_t}^{+} := {[\boldsymbol{y_{1, t}^T}^{+}, \dots, \boldsymbol{y_{N, t}^T}^{+}]}^T\boldsymbol{y_t}^{+} := {[\boldsymbol{y_{1, t}^T}^{+}, \dots, \boldsymbol{y_{N, t}^T}^{+}]}^T, 
${\Sigma_{t}} := {diag(\Sigma_{1, t}^T, \dots, \Sigma_{N, t}^T)}^T$. 
% % {\Sigma_{t}}^+ := {[{\Sigma_{1, t}^T}^+, \dots, {\Sigma_{N, t}^T}^+]}^T{\Sigma_{t}}^+ := {[{\Sigma_{1, t}^T}^+, \dots, {\Sigma_{N, t}^T}^+]}^T, 
% % {\Sigma_{t}}^- := {[{\Sigma_{1, t}^T}^-, \dots, {\Sigma_{N, t}^T}^-]}^T{\Sigma_{t}}^- := {[{\Sigma_{1, t}^T}^-, \dots, {\Sigma_{N, t}^T}^-]}^T,
% \chi := \chi_1 * \dots * \chi_M\chi := \chi_1 * \dots * \chi_M, and U := U_1 * \dots * U_MU := U_1 * \dots * U_M.


\subsection{Optimized Objective}\label{3.3}
The goal of the \textit{Resource Allocation System} is to allocate the sensing resources of AMAVs by planning the AMAVs, so as to limit the localization error of BMAVs.
Specifically, given a finite time horizon $T$, we select a sequence of motion commands of AMAVs $\boldsymbol{u_{0:T-1}}$, to limit the localization error of BMAVs in $T$.
The localization error of BMAVs can be mathematically expressed as 
% \begin{equation}
% \psi(T) := \sum_{t=1}^T\left(E\left[{||\boldsymbol{y_t}-\boldsymbol{\widehat{y}_t}||}^2\right]\right),
% \label{le}
% \end{equation}
$\psi(T) := \sum_{t=1}^T(E[{||\boldsymbol{y_t}- \boldsymbol{\widehat{y}_t}||}^2])$,
which is the sum of mean squared error (MSE) of $\boldsymbol{\widehat{y}_t}$.


% However, to calculate $\psi$, it is necessary to use the actual locations of BMAVs, and due to its own limited abilities and the lack of external localization infrastructure, the BMAVs cannot obtain actual locations.
% Under this limitation, we cannot guide the planning of AMAVs to allocate sensing resources by minimizing $\psi$.
% We found that the $\psi$ measures the quality of BMAVs' location estimations. 
% To solve the above problem, we would like to utilize a measure of information to reflect the quality of location estimations. 
% There are a variety of choices proposed in \cite{ucinski2004optimal} and for concreteness, we choose to optimize the trace of the covariance matrix of BMAVs’ location estimations which is theoretically appealing.
% This objective can be mathematically expressed as follows,
% \begin{equation}
% \xi(T) := \sum_{t=1}^T\left(tr\left(\Sigma_t\right)\right),
% \label{ob}
% \end{equation}
% which is an indication of the uncertainty of the BMAVs' location estimations. 
% The lower the indication the better the certainty of the location estimation is, and vice versa.


% The details can refer to Appendix \ref{MSE}.
% When the sensing resources are allocated, \xi\xi and \psi\psi decreases, and vice versa. 


To compute $\psi$, we require the actual locations of BMAVs, which are not obtainable due to their limited abilities and the absence of external localization infrastructure.
As a result, minimizing $\psi$ cannot guide the sensing resources allocation of AMAVs. 
Instead, we opt to optimize a measure of information which reflects the quality of BMAVs' location estimations.
Specifically, we choose to optimize the trace of the covariance matrix of BMAVs' location estimations \cite{ucinski2004optimal}, which can be mathematically expressed as 
% \begin{equation}
% \xi(T) := \sum_{t=1}^T\left(tr\left(\Sigma_t\right)\right).
% \label{ob}
% \end{equation}
$\xi(T) := \sum_{t=1}^T(tr(\Sigma_t)).$
This objective measures the uncertainty of location estimations, a lower value indicates greater certainty and vice versa.

\subsection{Problem Formulation}\label{3.4}
% In order to optimize the trace of the covariance matrix of BMAVs’ location estimation within the finite time horizon $T$, the \textit{Resource Allocation System} needs to consider the motion command of each AMAV within $T$. 
% Therefore, the mathematical formulation of the sensing resource allocation problem within a finite time horizon $T$ is defined as,
% \begin{equation}
% \min _{\boldsymbol{u_0}, \ldots, \boldsymbol{u_{T-1}}} \xi(T) = \sum_{t=1}^T\left(tr\left(\Sigma_t\right)\right),
% \end{equation}
% \begin{align}
%     \text { s.t. }
%     & \boldsymbol{x_{t+1}} = f(\boldsymbol{x_{t}}, \boldsymbol{u_{t}}), t \in \{0,\dots, T-1\} \\
%     & 0 \leq x_{j, t}^1, y_{i, t}^1 \leq L, \notag \\
%     & \quad j \in \{0,\dots, N\}, i \in \{0,\dots, M\}, t\in\{0,\dots, T-1\} \\
%     & 0 \leq x_{j, t}^2, y_{i, t}^2 \leq W, \notag \\
%     & \quad j \in \{0,\dots, N\}, i \in \{0,\dots, M\}, t\in\{0,\dots, T-1\} \\
%     & \Sigma_{t+1}=\rho_{t+1}^e\left(\rho_t^p\left(\Sigma_t\right), \boldsymbol{x}_{t+1}\right), t\in\{0,\dots, T-1\}.
% \end{align}
% where $\rho_t^e\left(\Sigma, \boldsymbol{x}\right)$ is the correction step, and $\rho_{t+1}^p$ is the prediction step. The detail of the two steps will be further introduced in Section \ref{4}-B. This problem is a deterministic optimization problem according to \cite{atanasov2014information}, and the Kalman Filter is the optimal estimator.

To optimize the trace of the covariance matrix of BMAVs’ location estimation within a finite time horizon $T$, the \textit{Resource Allocation System} must consider the motion commands of each AMAV within that horizon.
The corresponding mathematically formulated sensing resource allocation problem is given by,
\begin{equation}
\min _{\boldsymbol{u_0}, \ldots, \boldsymbol{u_{T-1}}} \xi(T) = \sum_{t=1}^T\left(tr\left(\Sigma_t\right)\right),
\end{equation}
\text {\centerline{s.t.} }
\begin{align}
    & \boldsymbol{x_{t+1}} = f(\boldsymbol{x_{t}}, \boldsymbol{u_{t}}), t \in \{0,\dots, T-1\} \\
    & 0 \leq x_{j, t}^1, y_{i, t}^1 \leq L, \\
    & \quad j \in \{0,\dots, N\}, i \in \{0,\dots, M\}, t\in\{0,\dots, T-1\} \notag \\
    & 0 \leq x_{j, t}^2, y_{i, t}^2 \leq W, \\
    & \quad j \in \{0,\dots, N\}, i \in \{0,\dots, M\}, t\in\{0,\dots, T-1\} \notag \\
    & \Sigma_{t+1}=\rho_{t+1}^e\left(\rho_t^p\left(\Sigma_t\right), \boldsymbol{x}_{t+1}\right), t\in\{0,\dots, T-1\}.
\label{problem}
\end{align}
The correction and prediction steps $\rho_t^e\left(\Sigma, \boldsymbol{x}\right)$ and $\rho_{t+1}^p$ respectively will be explained further in Section \ref{4}-B.



\begin{figure}[t]
    \centering
        \includegraphics[width=0.8\columnwidth]{Figs/observation.pdf}
    \caption{The observation model of AMAV. The observation angle of the visual sensor is $\phi$ and $r_m$ is the maximum distance that the sensor can observe. The FOV of $A_j$ is $F_{j, t}$. At time $t$, the noisy measurement generated by $A_j$ for $B_i$ consists of range $r_{i, j, t}$ and bearing $\alpha_{i, j, t}$.}
    \label{observation}
    \vspace{-0.4cm}
\end{figure} 
